Sample Efficient Reinforcement Learning via Low-Rank Matrix Estimation

We consider the question of learning $Q$-function in a sample efficient manner for reinforcement learning with continuous state and action spaces under a generative model. If $Q$-function is Lipschitz continuous, then the minimal sample complexity for estimating $\epsilon$-optimal $Q$-function is known to scale as ${\Omega}(\frac{1}{\epsilon^{d_1+d_2 +2}})$ per classical non-parametric learning theory, where $d_1$ and $d_2$ denote the dimensions of the state and action spaces respectively. The $Q$-function, when viewed as a kernel, induces a Hilbert-Schmidt operator and hence possesses square-summable spectrum. This motivates us to consider a parametric class of $Q$-functions parameterized by its "rank" $r$, which contains all Lipschitz $Q$-functions as $r \to \infty$. As our key contribution, we develop a simple, iterative learning algorithm that finds $\epsilon$-optimal $Q$-function with sample complexity of $\widetilde{O}(\frac{1}{\epsilon^{\max(d_1, d_2)+2}})$ when the optimal $Q$-function has low rank $r$ and the discounting factor $\gamma$ is below a certain threshold. Thus, this provides an exponential improvement in sample complexity. To enable our result, we develop a novel Matrix Estimation algorithm that faithfully estimates an unknown low-rank matrix in the $\ell_\infty$ sense even in the presence of arbitrary bounded noise, which might be of interest in its own right. Empirical results on several stochastic control tasks confirm the efficacy of our "low-rank" algorithms.

==> alg_rank1.tex <==
	\begin{algorithm}[H]
	\begin{algorithmic}[1]
	\STATE {\bfseries initialization:} $Q^{(0)}(s,a)$  and a corresponding $V^{(0)}(s) = \max_{a\in\mA}Q^{(0)}(s,a)$. 
		\FOR{$t = 1,2, \dots, T$}{
		\STATE discretize $\mS$ and $\mA$ into $\mS^{(t)} = \beta^{(t)}\textrm{-net of }\mS \textrm{ and } \mA^{(t)} = \beta^{(t)}\textrm{-net of }\mA.$
		\STATE randomly sample an anchor state $s^\dagger\in\mS^{(t)}$ and an anchor action $a^\dagger \in \mA^{(t)}$, and let
		\begin{equation*}
		\vspace{-0.03in}
		    \Omega^{(t)} = \big\{(s^\dagger, a)\big\}_{a\in\mA^{(t)}} \bigcup \{(s, a^\dagger)\big\}_{s\in\mS^{(t)}}
		    \vspace{-0.1in}
		\end{equation*}
		\FOR{$(s,a)\in\Omega^{(t)}$}{
		\STATE query the generative model to sample $C^{(t)}$ independent transitions $\{(s,a,s_i')\}_{i=1}^{C^{(t)}}$:
		\vspace{-0.05in}
		\begin{equation*}
		\label{eq:alg:generic:lookahead}
		    \hat{Q}^{(t)}(s,a) = R(s,a) + \gamma \cdot \frac{1}{C^{(t)}}\sum_{i=1}^{C^{(t)}}V^{(t-1)}(s'_i).
		    \vspace{-0.1in}
		\end{equation*}
		}
		\ENDFOR
		\STATE Complete the matrix:
		\vspace{-0.05in}
		\begin{equation*}
		    \bar{Q}^{(t)}(s,a) = \frac{\hat{Q}^{(t)}(s,a^\dagger) \hat{Q}^{(t)}(s^\dagger,a)}{\hat{Q}^{(t)}(s^\dagger,a^\dagger)},\:\forall\:(s,a)\in \mS^{(t)}\times \mA^{(t)}. 
		    \vspace{-0.13in}
		\end{equation*}
		
		\STATE 
		\vspace{-0.03in}
		\begin{align*}
		    Q^{(t)}(s,a) &= \textrm{Nearest Neighbor}\big(\{\bar{Q}^{(t)}(s,a)\}_{(s,a)\in \mS^{(t)}\times \mA^{(t)}}\big), \:\forall\: (s,a)\in\mS\times\mA,\\
		    V^{(t)}(s,a) &= \max_{a\in\mA}Q^{(t)}(s,a), \:\forall\: s\in\mS.
		    \vspace{-0.05in}
		\end{align*}
		}
		\ENDFOR
		\STATE {\bfseries Output:} $Q$-value oracle $Q^{(T)}$.
	
		%\vspace{10pt}
		\caption{Low-rank Reinforcement Learning: Rank-1}
			\label{alg:rank-1}
		\end{algorithmic}
	\end{algorithm}

==> alg_rank2.tex <==
	\begin{algorithm}[H]
	\begin{algorithmic}[1]
	\STATE {\bfseries initialization:} $Q^{(0)}(s,a)$  and a corresponding $V^{(0)}(s) = \max_{a\in\mA}Q^{(0)}(s,a)$. 
		\FOR{$t = 1,2, \dots, T$}{
		\STATE discretize $\mS$ and $\mA$ into $\mS^{(t)} = \beta^{(t)}\textrm{-net of }\mS \textrm{ and } \mA^{(t)} = \beta^{(t)}\textrm{-net of }\mA.$
		\STATE update $\mS$ and $\mA$ to contain the anchor states and actions if not included:
		\begin{equation*}
		\vspace{-0.03in}
		    \mS^{(t)}\leftarrow   \mS^{(t)}\bigcup \{s^\dagger_1,s^\dagger_2\}\:\textrm{ and }\: \mA^{(t)}\leftarrow   \mA^{(t)}\bigcup \{a^\dagger_1,a^\dagger_2\}
		    \vspace{-0.15in}
		\end{equation*}
		\STATE let
		\begin{equation*}
		\vspace{-0.03in}
		    \Omega^{(t)} = \big\{(s^\dagger, a)\big\}_{s^\dagger\in\{s^\dagger_1,s^\dagger_2\},a\in\mA^{(t)}}  \bigcup \{(s, a^\dagger_1)\big\}_{{s\in\mS^{(t)}},{a^\dagger\in\{a^\dagger_1,a^\dagger_2\}}}.
		    \vspace{-0.1in}
		\end{equation*}
		\FOR{$(s,a)\in\Omega^{(t)}$}{
		\STATE query the generative model to sample $C^{(t)}$ independent transitions $\{(s,a,s_i')\}_{i=1}^{C^{(t)}}$:
		\vspace{-0.05in}
		\begin{equation*}
		\label{eq:alg:generic:lookahead}
		    \hat{Q}^{(t)}(s,a) = R(s,a) + \gamma\cdot \frac{1}{C^{(t)}}\sum_{i=1}^{C^{(t)}}V^{(t-1)}(s'_i).
		    \vspace{-0.1in}
		\end{equation*}
		}
		\ENDFOR
		\STATE Complete the matrix:
		\vspace{-0.05in}
		\begin{equation*}
		    \bar{Q}^{(t)}(s,a) = \frac{
		    \begin{bmatrix}
\hat{Q}^{(t)}(s,a^\dagger_1) & \hat{Q}^{(t)}(s,a^\dagger_2)
\end{bmatrix}
\begin{bmatrix}
\hat{Q}^{(t)}(s_2^\dagger,a^\dagger_2) & -\hat{Q}^{(t)}(s^\dagger_1,a^\dagger_2)\\
-\hat{Q}^{(t)}(s^\dagger_2,a^\dagger_1) & \hat{Q}^{(t)}(s^\dagger_1,a^\dagger_1)
\end{bmatrix}
\begin{bmatrix}
\hat{Q}^{(t)}(s^\dagger_1,a) \\
\hat{Q}^{(t)}(s^\dagger_2,a)
\end{bmatrix}
}{\hat{Q}^{(t)}(s^\dagger_1,a^\dagger_1)\hat{Q}^{(t)}(s^\dagger_2,a^\dagger_2) - \hat{Q}^{(t)}(s^\dagger_2,a^\dagger_1)\hat{Q}^{(t)}(s^\dagger_1,a^\dagger_2)}
		    \vspace{-0.13in}
		\end{equation*}
		
		\STATE 
		\vspace{-0.03in}
		\begin{align*}
		    Q^{(t)}(s,a) &= \textrm{Nearest Neighbor}\big(\{\bar{Q}^{(t)}(s,a)\}_{(s,a)\in \mS^{(t)}\times \mA^{(t)}}\big), \:\forall\: (s,a)\in\mS\times\mA,\\
		    V^{(t)}(s,a) &= \max_{a\in\mA}Q^{(t)}(s,a), \:\forall\: s\in\mS.
		    \vspace{-0.05in}
		\end{align*}
		}
		\ENDFOR
		\STATE {\bfseries Output:} $Q$-value oracle $Q^{(T)}$.
	
		%\vspace{10pt}
		\caption{Low-rank Reinforcement Learning: Rank-2}
			\label{alg:rank-2}
		\end{algorithmic}
	\end{algorithm}

==> alg_rankr.tex <==
	\begin{algorithm}[H]
	\begin{algorithmic}[1]
	\STATE {\bfseries initialization:} $Q^{(0)}(s,a)$  and a corresponding $V^{(0)}(s) = \max_{a\in\mA}Q^{(0)}(s,a)$. 
		\FOR{$t = 1,2, \dots, T$}{
		\STATE discretize $\mS$ and $\mA$ into $\mS^{(t)} = \beta^{(t)}\textrm{-net of }\mS \textrm{ and } \mA^{(t)} = \beta^{(t)}\textrm{-net of }\mA.$
		\STATE update $\mS$ and $\mA$ to contain the anchor states and actions if not included:
		\begin{equation*}
		\vspace{-0.03in}
		    \mS^{(t)}\leftarrow   \mS^{(t)}\bigcup \{s^\dagger_1,s^\dagger_2,\dots,s^\dagger_r\}\:\textrm{ and }\: \mA^{(t)}\leftarrow   \mA^{(t)}\bigcup \{a^\dagger_1,a^\dagger_2,\dots, a^\dagger_r\}
		    \vspace{-0.15in}
		\end{equation*}
		\STATE let
		\begin{equation*}
		\vspace{-0.03in}
		    \Omega^{(t)} = \big\{(s^\dagger, a)\big\}_{s^\dagger\in\{s^\dagger_1,s^\dagger_2,\dots, s^\dagger_r\},a\in\mA^{(t)}}  \bigcup \{(s, a^\dagger_1)\big\}_{{s\in\mS^{(t)}},{a^\dagger\in\{a^\dagger_1,a^\dagger_2,\dots, a^\dagger_r\}}}.
		    \vspace{-0.1in}
		\end{equation*}
		\FOR{$(s,a)\in\Omega^{(t)}$}{
		\STATE query the generative model to sample $C^{(t)}$ independent transitions $\{(s,a,s_i')\}_{i=1}^{C^{(t)}}$:
		\vspace{-0.05in}
		\begin{equation*}
		\label{eq:alg:generic:lookahead}
		    \hat{Q}^{(t)}(s,a) = R(s,a) + \gamma\cdot \frac{1}{C^{(t)}}\sum_{i=1}^{C^{(t)}}V^{(t-1)}(s'_i).
		    \vspace{-0.1in}
		\end{equation*}
		}
		\ENDFOR
		\STATE Complete the matrix:
		\vspace{-0.05in}
		\begin{equation*}
		    \bar{Q}^{(t)}(s,a) = {
		    \begin{bmatrix}
\hat{Q}^{(t)}(s,a^\dagger_1) & \hat{Q}^{(t)}(s,a^\dagger_2) &\cdots &\hat{Q}^{(t)}(s,a^\dagger_r)
\end{bmatrix}
\big(\hat{\mathbb{Q}}^{(t),\dagger}\big)^{-1}
% \begin{bmatrix}
% \hat{Q}^{(t)}(s_2^\dagger,a^\dagger_2) & -\hat{Q}^{(t)}(s^\dagger_1,a^\dagger_2)\\
% -\hat{Q}^{(t)}(s^\dagger_2,a^\dagger_1) & \hat{Q}^{(t)}(s^\dagger_1,a^\dagger_1)
% \end{bmatrix}
\begin{bmatrix}
\hat{Q}^{(t)}(s^\dagger_1,a) \\
\hat{Q}^{(t)}(s^\dagger_2,a)\\
\vdots\\
\hat{Q}^{(t)}(s^\dagger_r,a)

\end{bmatrix}
}
		    \vspace{-0.13in}
		\end{equation*}
		
		\STATE 
		\vspace{-0.03in}
		\begin{align*}
		    Q^{(t)}(s,a) &= \textrm{Nearest Neighbor}\big(\{\bar{Q}^{(t)}(s,a)\}_{(s,a)\in \mS^{(t)}\times \mA^{(t)}}\big), \:\forall\: (s,a)\in\mS\times\mA,\\
		    V^{(t)}(s,a) &= \max_{a\in\mA}Q^{(t)}(s,a), \:\forall\: s\in\mS.
		    \vspace{-0.05in}
		\end{align*}
		}
		\ENDFOR
		\STATE {\bfseries Output:} $Q$-value oracle $Q^{(T)}$.
	
		%\vspace{10pt}
		\caption{Low-rank Reinforcement Learning: Rank-$r$}
			\label{alg:rank-r}
		\end{algorithmic}
	\end{algorithm}

==> rank1.tex <==
\section{Warm-up: Rank-$1$ Reinforcement Learning}
\label{sec:rank1}

%{\bf Model Assumption}
We consider a simple yet concrete setup where $Q^*$ has rank $1$, i.e., there exist $f: \mS \to \RR$ and $g: \mA \to \RR$ such that for all $(s,a) \in \mS \times \mA$,
$
    Q^*(s,a) = f(s) \cdot g(a).
$
For a simpler exposition, in this section only, we make an additional assumption that $R(s,a)\in[R_{\min}, R_{\max}]$ where $ R_{\min} > 0$ for all $(s,a) \in \mS \times \mA$. Hence, for any policy, $Q(s,a) \geq V_{\min} = \frac{R_{\min}}{1 - \gamma}$. 






{\bf Algorithmic Choices Developed} %\label{sec:alg_rank1} 
Intuitively, being rank-$1$ implies that $Q^*$ intrinsically has only "one-dimensional" freedom. Consider discretized set $\mS^{(t)}\times \mA^{(t)}$ and the $|\mS^{(t)}|\times |\mA^{(t)}|$ matrix, $Q^*(\mS^{(t)},\mA^{(t)})$, obtained by restricting the $Q^*$-function on the discretized set. Then $Q^*(\mS^{(t)},\mA^{(t)})$ can be represented as $FG$, where $F\in\mathbb{R}^{|\mS^{(t)}|\times 1}$ is a column vector with entries $\{f(s)\}_{s\in\mS^{(t)}}$ and   $G\in\mathbb{R}^{1\times|\mA^{(t)}|}$ is a row vector with entries $\{g(a)\}_{a\in\mA^{(t)}}$. Therefore, estimating $Q^*(\mS^{(t)},\mA^{(t)})$ amounts to understanding the one-dimensional "column space" and the one-dimensional "row space". This motivates us to explore \emph{one} entire row and \emph{one} entire column. Formally,
% \red{DG: For statistical/numerical stability, we should choose the anchor points in a refined fashion so that $\big| Q^*(s^{\sharp}, a^{\sharp} \big|$ is not too small. }
\begin{itemize}
    \item
    Choice of exploration set $\Omega^{(t)}$:
    At each $t =1, \ldots, T$, choose an anchor state $s^{\sharp} \in \mS^{(t)}$ and an anchor action $a^{\sharp} \in \mA^{(t)}$. 
    Then let $\Omega^{(t)} = \{ (s,a) \in \mS^{(t)} \times \mA^{(t)}: s = s^{\sharp} \text{ or } a = a^{\sharp} \}$.
    
    \item
    Matrix Estimation subroutine:
    For $(s,a) \in \mS^{(t)} \times \mA^{(t)}$, we let
    $ %\begin{equation}\label{eqn:me_rank1}
        \bar{Q}^{(t)}(s,a) = \frac{\hat{Q}^{(t)}(s,a^\sharp) \hat{Q}^{(t)}(s^\sharp,a)}{\hat{Q}^{(t)}(s^\sharp,a^\sharp)}.
    $ %\end{equation}
\end{itemize}
% Rule to choose $\beta^{(t)}$
% Rule to choose $N^{(t)}$
Note that $|\Omega^{(t)}| = |\mS^{(t)}| + |\mA^{(t)}| - 1$, which is much smaller than $ | \mS^{(t)} | |\mA^{(t)}|$, the cardinality of the entire (discretized) state-action space at iteration $t$. 
%For better stability, it would better to choose "nice" $s^{\sharp}, a^{\sharp}$ such that $Q^*( s^{\sharp}, a^{\sharp} )$ is large:
%identifying only a single state and action that is good is often trivial in many tasks.

{\bf Theoretical Guarantees} The following proposition characterizes the performance of our choices.
%\label{subsec:rank1_theory}


\begin{prop}\label{prop:rank1}
    Let $\Omega^{(t)}$ and $\bar{Q}^{(t)}$ as described above.
    For any $\epsilon \leq \frac{1}{2} V_{\min}$, we have
    \begin{equation*}
        \max_{(s,a) \in \Omega^{(t)}} \big| \hat{Q}^{(t)}(s,a) - Q^*(s,a) \big| \leq \epsilon
        \quad\implies\quad
        \max_{(s,a) \in \mS^{(t)}\times \mA^{(t)}} \big| \bar{Q}^{(t)}(s,a) - Q^*(s,a) \big| \leq 7 \frac{R_{\max}}{R_{\min}} \epsilon.
    \end{equation*}
\end{prop}
That is, the simple procedure described above satisfies Assumption \ref{assu:me} with $C=1$ and $c_{\eta} = 7 \frac{R_{\max}}{R_{\min}}$. We remark that indeed it is possible to show a more general statement that for any $c\in[0,1)$, and any $\epsilon\leq cV_{\min}$, if $\max_{(s,a) \in \Omega^{(t)}} \big| \hat{Q}^{(t)}(s,a) - Q^*(s,a) \big| \leq \epsilon$, then $\max_{(s,a) \in \mS^{(t)}\times \mA^{(t)}} \big| \bar{Q}^{(t)}(s,a) - Q^*(s,a) \big| \leq \frac{3+c}{1-c}\frac{R_{\max}}{R_{\min}}$. We let $c = \frac{1}{2}$ in Proposition \ref{prop:rank1} for the convenience in exposition.

With Proposition \ref{prop:rank1} at hand, we can obtain the following theorem as a Corollary of Theorem \ref{thm:generic} for the rank-1 setup. The proof basically remains the same, and we only need to additionally verify $\max_{(s,a) \in \Omega^{(t)}} \big| \hat{Q}^{(t)}(s,a) - Q^*(s,a) \big| \leq \frac{1}{2} V_{\min}$ for all $t = 1, \ldots, T$ to use Proposition \ref{prop:rank1}.
% The proof is basically an instantiation of the generic proof of Theorem \ref{thm:generic}, and we will concisely summarize the key steps in Section \ref{subsec:rank1_theory}.




\begin{thm}
\label{thm:rank1}
    % Let there be a rank-1 MDP problem such that (i) $R(s,a) \in [R_{\min}, R_{\max}]$ for all $(s,a) \in \mS \times \mA$ where $R_{\min} > 0$ and (ii) $\gamma < \frac{R_{\min}}{14 R_{\max}}$. 
    % Suppose that we run Algorithm \ref{alg:generic} initialized at $Q^{(0)} \equiv 0$ to solve the MDP problem with the exploration and the matrix estimation steps as described above.
    
    Consider the rank-$1$ setting in this section. Suppose that we run  Algorithm \ref{alg:generic} with the exploration and the matrix estimation steps as described.% above.
    If $\gamma < \frac{R_{\min}}{14 R_{\max}}$, then the following holds.
    \begin{enumerate}
    \item
    For any $\delta > 0$,  we have 
    $%\begin{equation*}%\label{eqn:geom_rate}
        \sup_{ (s,a) \in \mS \times \mA } \big| Q^{(t)}(s,a) - Q^*(s,a) \big|
            \leq \big( \frac{14 R_{\max}}{R_{\min}} \gamma \big)^t V_{\max}
            $, $\forall\:t = 1, \dots, T,
    $ %\end{equation*}
    with probability at least $1 - \delta$ 
    by choosing algorithmic parameters $\beta^{(t)}, N^{(t)}$ appropriately.
    % $\beta^{(t)} = \frac{V_{\max}}{8L} \big( \frac{14 R_{\max}}{R_{\min}} \gamma \big)^t$, $N^{(t)} = 8 \big( \frac{14 R_{\max}}{R_{\min}} \gamma \big)^{-2(t-1)} \log\big(\frac{2 | \Omega^{(t)} | T}{\delta}\big)$ for $t = 1, \ldots, T$.
    
    \item
    For any $\epsilon > 0$ and $\delta > 0$, it suffices to set $T = \Theta( \log \frac{1}{\epsilon} )$ and use $\tilde{O}( \frac{1}{\epsilon^{d+2}} \cdot \log \frac{1}{\delta} )$ samples to achieve $\sup_{(s,a) \in \mS \times \mA} \big| Q^{(T)}(s,a) - Q^*(s,a) \big| \leq \epsilon$ with probability at least $1 - \delta$.
    \end{enumerate}
\end{thm}











% \section{Warm-up: Rank-$1$ Reinforcement Learning}
% With the generic results at hand, we now provide explicit sampling scheme for selecting the subset $\Omega^{(t)}$  and the corresponding algorithms for the matrix estimation oracle. The main goal is to demonstrate a practical and provable oracle that satisfying the desired performance guarantees, i.e., Assumption \ref{assu:me}, under proper conditions. To develop the intuition and facilitate a better understanding, let us start with the rank-1 case.

% Throughout this section, we consider reinforcement learning when $Q^*$ is rank-1. That is, there exist some functions $f:\mS\rightarrow \mathbb{R}$ and $g:\mA\rightarrow\mathbb{R}$ such that 
% \begin{equation*}
%     Q^*(s,a) = f(s)\cdot g(a).
% \end{equation*}
% In Section \ref{subsec:rank1_alg}, we first provide intuitions for developing a suitable matrix estimation oracle under this setting and then introduce the full algorithm. Provable guarantees are given in Section \ref{subsec:rank1_theory}.

% \subsection{Algorithm}
% \label{subsec:rank1_alg}

% \input{alg_rank1}
% \subsection{Theoretical Guarantees}
% \label{subsec:rank1_theory}

% We assume that $R\in[R_{\min}, R_{\max}]$
% \begin{prop}
% \label{prop:rank1}
% Fix an iteration $t$. Suppose that 
% \begin{equation*}
%     |\hat{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \epsilon, \:\forall\:(s,a)\in\Omega^{(t)},
% \end{equation*}
% where $\epsilon \leq cV_{\min}$ for some constant $c\in(0,1)$. Then,
% \begin{equation}
%     |\bar{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \eta\cdot \epsilon, \:\forall\:(s,a)\in \mS^{(t)}\times\mA^{(t)},
% \end{equation}
% where $\eta = \frac{(3+c)R_{\max}}{(1-c)R_{\min}}$.
% \end{prop}
% With Proposition \ref{prop:rank1}, we can apply our meta theorem, Theorem \ref{thm:generic}, to derive the convergence and sample complexity results as stated in the following. The proof is basically an instantiation of the generic proof of Theorem \ref{thm:generic}, and we will concisely summarize the key steps in Section \ref{subsec:rank1_theory}.

% \begin{thm}
% \label{thm:rank-1}
%     %Consider running Algorithm \ref{alg:generic} for $T$ iterations. 
%     Suppose that Assumption \ref{assu:lipschitz} hold. Then, for any MDP problem where $\gamma$ satisfies
%     \begin{equation}
%     \label{eq:thm:rank-1:gamma}
%     \gamma <\min\Big\{c,\:\frac{1-c}{3+c}\Big\}\cdot\frac{R_{\min}}{R_{\max}}
%     \end{equation}
%     for some constant $c\in(0,1)$, we have the following guarantees for Algorithm \ref{alg:rank-1}: 
    
%     \begin{enumerate}
%         \item (Convergence) For any $\alpha\in\big(\gamma\frac{(3+c)R_{\max}}{(1-c)R_{\min}}, 1\big)$, there exist appropriate algorithmic parameters such that with probability at least $1-\delta$
%         \begin{equation}
%             |Q^{(T)}(s,a) - Q^*(s,a)|\leq \alpha^TV_{\max},\:\forall\:(s,a)\in\mS\times\mA.
%         \end{equation}
%     \item (Sample Complexity) Therefore, to achieve an $\epsilon$ error for the $Q$-value with probability at least $1-\delta$, i.e., $|Q^{(T)}-Q^*|_{\max}\leq\epsilon$, the number of iterations $T=\Theta\big(\log\frac{1}{\epsilon}\big)$ and the total number of samples needed is
%     \begin{equation}
%         \widetilde{O}\Big(\epsilon^{-(2+d)}\cdot\log\frac{1}{\delta}\Big).
%     \end{equation}
%     \end{enumerate}
% \end{thm}

% \subsection{Proofs}
% \begin{proof}[Proof of Proposition \ref{prop:rank1}]
% First, we note that $Q^*$ can be rewritten as 
% \begin{equation*}
%     Q^*(s,a) = \frac{Q^*(s, a^\dagger)Q^*(s^\dagger,a)}{Q^*(s^\dagger,a^\dagger)}.
% \end{equation*}
% To see this, notice that $Q^*$ being rank-1 implies that the numerator equals to $f(s)g(a^\dagger)f(s^\dagger)g(a)$ and the denominator equals to $f(s^\dagger)g(a^\dagger)$.

% Now, note that by assumption in the proposition, for $(s,a)\in\Omega^{(t)}$,
% \begin{equation*}
%     Q^*(s,a) - \epsilon \leq \hat{Q}^{(t)}(s,a) \leq Q^*(s,a) + \epsilon.
% \end{equation*}
% Since $Q^*(s,a)\geq V_{\min}$, the previous equation implies the following multiplicative error bound:
% \begin{equation}
% \label{eq:rank1:prop:proof:multi}
%   \big(1-\frac{\epsilon}{V_{\min}}\big) Q^*(s,a)  \leq \hat{Q}^{(t)}(s,a) \leq \big(1+\frac{\epsilon}{V_{\min}}\big)Q^*(s,a).
% \end{equation}
% Also, we note that because $\epsilon\leq cV_{\min}$, the lower bound $(1-\epsilon/V_{\min})Q^*(s,a)\geq (1-c)Q^*(s,a) > 0$. We now derive the error guarantees for $\bar{Q}^{(t)}(s,a)$. Recall that for $(s,a)\in\mS^{(t)}\times \mA^{(t)}$, the estimator $\bar{Q}^{(t)}$ is
% 	\begin{equation*}
% 		    \bar{Q}^{(t)}(s,a) = \frac{\hat{Q}^{(t)}(s,a^\dagger) \hat{Q}^{(t)}(s^\dagger,a)}{\hat{Q}^{(t)}(s^\dagger,a^\dagger)}.
% 		\end{equation*}
% Combining this with the error bound Eq.~(\ref{eq:rank1:prop:proof:multi}), we obtain that
% \begin{align*}
%   &\frac{(1-\epsilon/V_{\min})^2}{(1+\epsilon/V_{\min})}\cdot\frac{Q^*(s, a^\dagger)Q^*(s^\dagger,a)}{Q^*(s^\dagger,a^\dagger)}\leq  \bar{Q}^{(t)}(s,a)\leq\frac{(1+\epsilon/V_{\min})^2}{(1-\epsilon/V_{\min})}\cdot\frac{Q^*(s, a^\dagger)Q^*(s^\dagger,a)}{Q^*(s^\dagger,a^\dagger)}.
% \end{align*}
% That is,
% \begin{equation}
% \label{eq:rank1:prop:proof:barQ}
%     \Big(\frac{(1-\epsilon/V_{\min})^2}{(1+\epsilon/V_{\min})}-1\Big)Q^*(s,a)\leq  \bar{Q}^{(t)}(s,a)- Q^*(s,a)\leq\Big(\frac{(1+\epsilon/V_{\min})^2}{(1-\epsilon/V_{\min})}-1\Big)Q^*(s,a)
% \end{equation}
% In the following, we simplify the lower and upper bounds in Eq.~(\ref{eq:rank1:prop:proof:barQ}) to derive the desired bounds in the proposition. Let us consider first the upper bound.
% \begin{align*}
%     \Big(\frac{(1+\epsilon/V_{\min})^2}{(1-\epsilon/V_{\min})}-1\Big)Q^*(s,a) & =\Big(\frac{3\frac{\epsilon}{V_{\min}} + \frac{\epsilon^2}{V_{\min}^2}}{1-\frac{\epsilon}{V_{\min}}}\Big)Q^*(s,a)\\
%     & = \frac{\epsilon}{V_{\min}}\Big(\frac{3+\frac{\epsilon}{V_{\min}}}{1-\frac{\epsilon}{V_{\min}}}\Big)Q^*(s,a)\\
%     & \leq \frac{V_{\max}}{V_{\min}} \Big(\frac{3+\frac{\epsilon}{V_{\min}}}{1-\frac{\epsilon}{V_{\min}}}\Big)\cdot\epsilon\\
%     &\leq  \frac{R_{\max}}{R_{\min}} \Big(\frac{3+c}{1-c}\Big)\cdot\epsilon,
% \end{align*}
% where the last inequality follows from the following facts: (1) $\frac{V_{\max}}{V_{\min}}= \frac{R_{\max}/(1-\gamma)}{R_{\min} /(1-\gamma}= \frac{R_{\max}}{R_{\min}}$; (2) $\epsilon\leq cV_{\min}$ by assumption and the function $\frac{3+x}{1-x}$ is increasing in $x\in[0,1)$. 

% We now move to the lower bound in Eq.~(\ref{eq:rank1:prop:proof:barQ}):
% \begin{align*}
%      \Big(\frac{(1-\epsilon/V_{\min})^2}{(1+\epsilon/V_{\min})}-1\Big)Q^*(s,a) & =\Big(\frac{-3\frac{\epsilon}{V_{\min}} + \frac{\epsilon^2}{V_{\min}^2}}{1+\frac{\epsilon}{V_{\min}}}\Big)Q^*(s,a)\\
%      & = \frac{\epsilon}{V_{\min}}\Big(\frac{\frac{\epsilon}{V_{\min}}-3}{\frac{\epsilon}{V_{\min}}+1}\Big)Q^*(s,a)\\
%      & \geq\frac{V_{\max}}{V_{\min}}\Big(\frac{\frac{\epsilon}{V_{\min}}-3}{\frac{\epsilon}{V_{\min}}+1}\Big)\epsilon\\
%      &\geq \frac{R_{\max}}{R_{\min}}\cdot(-3)\cdot\epsilon,
% \end{align*}
% where the inequalities follows from the following facts: (1) $Q^*(s,a)\leq V_{\max}$ and $\epsilon/V_{\min} - 3 < 0$; (2) the function $\frac{x -3}{x+1}$ is increasing and negative in $x\in[0,1)$.

% To summarize, per Eq.~(\ref{eq:rank1:prop:proof:barQ}), we have that
% \begin{equation*}
%     -3\frac{R_{\max}}{R_{\min}}\leq \bar{Q}^{(t)}(s,a) - Q^*(s,a)\leq \Big(\frac{3+c}{1-c}\Big)\frac{R_{\max}}{R_{\min}}\epsilon.
% \end{equation*}
% Therefore,
% \begin{align*}
%     |\bar{Q}^{(t)}(s,a) - Q^*(s,a)|&\leq\max\Big\{3,\frac{3+c}{1-c}\Big\}\frac{R_{\max}}{R_{\min}}\cdot\epsilon\\
%     & = \frac{(3+c)R_{\max}}{(1-c)R_{\min}}\cdot \epsilon.
% \end{align*}
% This completes the proof of the proposition.
% \end{proof}

% \begin{proof}[Proof of Theorem \ref{thm:rank-1}]
% As mentioned, from a high-level perspective, the proof is basically an instantiation of the generic proof for Theorem \ref{thm:generic} by replacing the assumption on the matrix estimation oracle (i.e., Assumption \ref{assu:me}) with the explicit guarantee in Proposition \ref{prop:rank1}. However, note that Proposition \ref{prop:rank1} holds only when the error $|\hat{Q}^{(t)}(s,a)-Q^*(s,a)|$ satisfies certain condition. This in return affects our choices of algorithmic parameters slightly. In the following, we provide this key modification of the generic proof to complete our arguments for Theorem \ref{thm:rank-1}.

% Recall that in Part I of the generic proof, by applying Lemma \ref{lem:one_step_lookahead}, we obtain that 
% for a state-action pair $(s,a)\in\Omega^{(t)}$, with probability $1- \xi$, the improve estimate $\hat{Q}^{(t)}(s,a)$ satisfies
% \begin{equation*}
% %\label{eq:proof:thm:generic:one_step}
%     |\hat{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \gamma(\lambda^{(t)} + B^{(t-1)}),
% \end{equation*}
% where we suppose that the error of $\hat{V}^{(t-1)}$ satisfies that 
% $||\hat{V}^{(t-1)}-V^*||_{\max} \leq B^{(t-1)}.$ For now, let us assume that the bound $B^{(t-1)}$ satisfies $B^{(t-1)}\leq V_{\max}$; we will see that this is easily implied by the choice of algorithmic parameters. Then, from the condition of Theorem \ref{thm:rank-1}, i.e., Eq.~(\ref{eq:thm:rank-1:gamma}) on $\gamma$, it is obvious that if we let 
% \begin{equation*}
%     \lambda ^{(t)}\leq \frac{cV_{\min}}{\gamma}-V_{\max},
% \end{equation*}
% then,
% \begin{equation*}
% %\label{eq:proof:thm:generic:one_step}
%     |\hat{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \gamma(\lambda^{(t)} + B^{(t-1)})\leq cV_{\min}.
% \end{equation*}
% In particular, this allows us to apply Proposition \ref{prop:rank1} to derive the error bound for $\bar{Q}^{(t)}$ after the matrix completion step. In the subsequent proof, we will condition on that $\lambda^{(t)}$ is selected such that  $\lambda ^{(t)}\leq \frac{cV_{\min}}{\gamma}-V_{\max}$ for all $t=1,\dots,T$. Therefore, we obtain that at iteration $t$, with probability at least $1-|\Omega^{(t)}|\times\xi$,
% \begin{equation*}
%     |\bar{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \gamma\eta(\lambda^{(t)}+B^{(t-1)}), \:\forall\:(s,a)\in\mS^{(t)} \times \mA^{(t)},
% \end{equation*}
% where 
% \begin{equation*}
%     \eta = \frac{(3+c)R_{\max}}{(3-c)R_{\min}}.
% \end{equation*}
% Finally, by the particular choice of $\Omega^{(t)}$ in Algorithm \ref{alg:rank-1}, i.e., $ \Omega^{(t)} = \big\{(s^\dagger, a)\big\}_{a\in\mA^{(t)}} \bigcup \{(s, a^\dagger)\big\}_{s\in\mS^{(t)}}$, we also have that $|\Omega^{(t)}|=O\big((\beta^{(t)})^{-d})$.

% For Part II of the generic proof, it is obvious that the recursive equation readily follows. That is, using the same definitions of $\varepsilon^{(t)}_Q$ and $\varepsilon^{(t)}_V$,
% \begin{align}
% \label{eq:thm:rank1:proof:recursion}
%   \varepsilon^{(t)}_Q 
%     & \leq  2L\beta^{(t)} + \gamma\eta\lambda^{(t)} + \gamma\eta \varepsilon_Q^{(t-1)} 
% \end{align}

% To select the algorithmic parameters, we follow the same reasoning as in Part III of the generic proof. Specifically, we prove by induction that
% \begin{equation*}
%     \varepsilon^{(t)}_Q\leq V_{\max}\alpha^t,
% \end{equation*}
% where we recall the conditions that $\alpha\in\big(\gamma\frac{(3+c)R_{\max}}{(1-c)R_{\min}}, 1\big)$.
% Note that this shall lead to the desired convergence result in Theorem \ref{thm:rank-1}. In addition, by using the fact that $\varepsilon^{(t)}_V\leq \varepsilon^{(t)}_Q$ (cf. Eq.~(\ref{eq:thm:generic:proof:varepsilonV})), the above equation also implies that $B^{(t)}\leq V_{\max}$ for each iteration $t$, which is desirable as mentioned previously. 

% Let us prove the result by induction. Notice that $\varepsilon^{(0)}_Q\leq V_{\max}$ holds trivially by setting $Q^{(0)}=0$. By induction, suppose that  $\varepsilon^{(t-1)}_Q\leq V_{\max}\alpha^{t-1}$, then from the recursive equation Eq.~(\ref{eq:thm:rank1:proof:recursion}), we would like to show that we could choose appropriate parameters such that
% \begin{align*}
%     \varepsilon^{(t)}_Q&\leq  2L\beta^{(t)} + \gamma\eta\lambda^{(t)} + \gamma\eta V_{\max}\alpha^{t-1} \nonumber\\
%     &\leq V_{\max}\alpha^{t}.
% \end{align*}
% Again, it is not hard to see that one could set the parameters $\beta^{(t)}$ and $\lambda^{(t)}$ to be such that
% \begin{align*}
%     2L\beta^{(t)} \leq \frac{\alpha-\gamma\eta}{2}V_{\max}\alpha^{t-1}\textrm{ and }\gamma\eta\lambda^{(t)}  \leq \frac{\alpha-\gamma\eta}{2}V_{\max}\alpha^{t-1}.
% \end{align*}
% Additionally, recall that previously in the proof, we have conditioned on that $\lambda ^{(t)}\leq \frac{cV_{\min}}{\gamma}-V_{\max}$. Therefore, to summarize, we can set the parameters to be 
% \begin{align}
%     \beta^{(t)} = \frac{\alpha-\gamma\eta}{4L}V_{\max}\alpha^{t-1}\textrm{ and }\lambda^{(t)}  = \min\Big\{\frac{cV_{\min}}{\gamma}-V_{\max}, \frac{\alpha-\gamma\eta}{2\gamma\eta}V_{\max}\alpha^{t-1}\Big\}. \label{eq:thm:rank1:proof:constants}
% \end{align}
% With these choices of $\beta^{(t)}$ and $\lambda^{(t)}$, we have that $\varepsilon^{(t)}_Q\leq V_{\max}\alpha^t$ and hence, completes the induction proof.

% Finally, the sample complexity follows exactly the same steps in Part IV of the generic proof. In particular, we note that to achieve $\varepsilon^{(T)}_Q\leq \epsilon$, we have $T=\Theta(\log\frac{1}{\epsilon})$ from the induction proof above. Furthermore, the choice of $\beta^{(t)}$ and $\lambda^{(t)}$ in Eq.~(\ref{eq:thm:rank1:proof:constants}) implies that $\beta^{(T)}=\Theta(\epsilon)$ and $\lambda^{(T)}=\Theta(\epsilon)$. The rest of the proof is the same, and this completes the proof of Theorem \ref{thm:rank-1}.
% \end{proof}

==> rank2.tex <==
\section{Rank-$2$ Reinforcement Learning}
% With the generic results at hand, we now provide explicit sampling scheme for selecting the subset $\Omega^{(t)}$  and the corresponding algorithms for the matrix estimation oracle. The main goal is to demonstrate a practical and provable oracle that satisfying the desired performance guarantees, i.e., Assumption \ref{assu:me}, under proper conditions. To develop the intuition and facilitate a better understanding, let us start with the rank-1 case.

Throughout this section, we consider reinforcement learning when $Q^*$ is rank-2. That is, there exist some functions $f:\mS\rightarrow \mathbb{R}$ and $g:\mA\rightarrow\mathbb{R}$ such that 
\begin{equation*}
    Q^*(s,a) = \sum_{i=1}^2f_i(s)\cdot g_i(a).
\end{equation*}
% In Section \ref{subsec:rank1_alg}, we first provide intuitions for developing a suitable matrix estimation oracle under this setting and then introduce the full algorithm. Provable guarantees are given in Section \ref{subsec:rank1_theory}.

\subsection{Algorithm}
\label{subsec:rank2_alg}

\input{alg_rank2}
\subsection{Theoretical Guarantees}
\label{subsec:rank2_theory}

For convenience, let us assume that $R\in[R_{\min}, R_{\max}]$ for the rank-1 case. This is not needed when we go to the general rank-$r$ algorithm
\begin{assumption}
\label{assu:rank2_c}
There exists a constant $c\in(0,1)$ such that the anchor states $\{s_1^\dagger,s_2^\dagger\}$ and anchor actions $\{a_1^\dagger,a_2^\dagger\}$ satisfy
    \begin{equation*}
        \frac{Q^*(s_1^\dagger,a_1^\dagger)Q^*(s_2^\dagger,a_2^\dagger)}{Q^*(s_2^\dagger,a_1^\dagger)Q^*(s_1^\dagger,a_2^\dagger)}\geq \frac{(1+c)^2 + \Delta}{(1-c)^2}
    \end{equation*}
    for some constant $\Delta > 0$.
    
% \begin{enumerate}
%     \item The discounting factor $\gamma \leq c\cdot\frac{R_{\min}}{R_{\max}}$.
%     \item The anchor states $\{s_1^\dagger,s_2^\dagger\}$ and anchor actions $\{a_1^\dagger,a_2^\dagger\}$ satisfy
%     \begin{equation*}
%         \frac{Q^*(s_1^\dagger,a_1^\dagger)Q^*(s_2^\dagger,a_2^\dagger)}{Q^*(s_2^\dagger,a_1^\dagger)Q^*(s_1^\dagger,a_2^\dagger)}\geq \frac{(1+c)^2 + \Delta}{(1-c)^2}
%     \end{equation*}
%     for some constant $\Delta > 0$.
% \end{enumerate}
\end{assumption}

\begin{lem}
\label{lem:rank2:unbiased}
Suppose that Assumption \ref{assu:rank2_c} holds. Then, for every $(s,a)\in\mS\times\mA$,
\begin{equation}
\label{eq:lem:rank2:unbias}
		    {Q}^*(s,a) = \frac{
		    \begin{bmatrix}
{Q}^*(s,a^\dagger_1) & {Q}^*(s,a^\dagger_2)
\end{bmatrix}
\begin{bmatrix}
{Q}^*(s_2^\dagger,a^\dagger_2) & -{Q}^*(s^\dagger_1,a^\dagger_2)\\
-{Q}^*(s^\dagger_2,a^\dagger_1) & {Q}^*(s^\dagger_1,a^\dagger_1)
\end{bmatrix}
\begin{bmatrix}
{Q}^*(s^\dagger_1,a) \\
{Q}^*(s^\dagger_2,a)
\end{bmatrix}
}{{Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) - {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2)}
		\end{equation}
\end{lem}

\begin{prop}
\label{prop:rank2}
Fix an iteration $t$ and suppose that Assumption \ref{assu:rank2_c} holds. If $\forall\:(s,a)\in\Omega^{(t)}$, the estimator $\hat{Q}$ satisfies $|\hat{Q}^{(t)}(s,a)|\leq V_{\max}$ and 
\begin{equation*}
    |\hat{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \epsilon,% \:\forall\:(s,a)\in\Omega^{(t)},
\end{equation*}
where $\epsilon \leq cV_{\min}$. Then,
\begin{equation}
    |\bar{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \eta\cdot \epsilon, \:\forall\:(s,a)\in \mS^{(t)}\times\mA^{(t)},
\end{equation}
where $\eta = \frac{40R_{\max}^4}{\Delta^2 R_{\min}^4}$.
\end{prop}
With Proposition \ref{prop:rank2}, we can again apply our meta theorem, Theorem \ref{thm:generic}, to derive the convergence and sample complexity results for the rank-2 case. The proof is exactly the same as the one for the rank-1 scenario except that we replace the rank-1 matrix estimation guarantee (Proposition \ref{prop:rank1}) with Proposition \ref{prop:rank2}, in particular, using $\eta = \frac{40R_{\max}^4}{\Delta^2R_{\min}^4}$ in the proof.
We hence state the resulting theorem in the following and omit its proof.

\begin{thm}
\label{thm:rank-2}
    %Consider running Algorithm \ref{alg:generic} for $T$ iterations. 
    Suppose that Assumption \ref{assu:lipschitz} and \ref{assu:rank2_c} hold. Then, for any MDP problem where $\gamma$ satisfies
    \begin{equation}
    \gamma <\min\Big\{c,\:\frac{\Delta^2}{40}\cdot\frac{R^3_{\min}}{ R^3_{\max}}\Big\}\cdot \frac{R_{\min}}{R_{\max}},
    \end{equation}
     we have the following guarantees for Algorithm \ref{alg:rank-2}: 
    
    \begin{enumerate}
        \item (Convergence) For any $\alpha\in\big(\gamma\frac{40R_{\max}^4}{\Delta^2 R_{\min}^4}, 1\big)$, there exist appropriate algorithmic parameters such that with probability at least $1-\delta$
        \begin{equation}
            |Q^{(T)}(s,a) - Q^*(s,a)|\leq \alpha^TV_{\max},\:\forall\:(s,a)\in\mS\times\mA.
        \end{equation}
    \item (Sample Complexity) Therefore, to achieve an $\epsilon$ error for the $Q$-value with probability at least $1-\delta$, i.e., $|Q^{(T)}-Q^*|_{\max}\leq\epsilon$, the number of iterations $T=\Theta\big(\log\frac{1}{\epsilon}\big)$ and the total number of samples needed is
    \begin{equation}
        \widetilde{O}\Big(\epsilon^{-(2+d)}\cdot\log\frac{1}{\delta}\Big).
    \end{equation}
    \end{enumerate}
\end{thm}

\subsection{Proofs}
\begin{proof}[Proof of Lemma \ref{lem:rank2:unbiased}]
One straightforward approach to prove Lemma \ref{lem:rank2:unbiased} is to expand the R.H.S. of Eq.~(\ref{eq:lem:rank2:unbias}) using the rank-2 expansion, i.e., $Q^*(s,a)=\sum_{i=1}^2f_i(s)\cdot g_i(a)$, and then work out the algebra. This appears to involve a lot of tedious calculations. Here, we present an alternative proof.

Consider the following $2\times 2$ matrix
\begin{equation*}
   Q^\dagger \triangleq \begin{bmatrix}
{Q}^*(s_1^\dagger,a^\dagger_1) & {Q}^*(s^\dagger_1,a^\dagger_2)\\
{Q}^*(s^\dagger_2,a^\dagger_1) & {Q}^*(s^\dagger_2,a^\dagger_2).
\end{bmatrix}
\end{equation*}
By assumption, the determinant 
\begin{equation*}
    \textrm{det}(Q^\dagger) = {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) - {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2) > 0,
\end{equation*}
and hence $Q^\dagger$ is invertible. For a $2\times 2 $ matrix, one can explicitly write out the analytical solution for inversion, which gives us
\begin{equation*}
    (Q^\dagger)^{-1} =  \frac{
\begin{bmatrix}
{Q}^*(s_2^\dagger,a^\dagger_2) & -{Q}^*(s^\dagger_1,a^\dagger_2)\\
-{Q}^*(s^\dagger_2,a^\dagger_1) & {Q}^*(s^\dagger_1,a^\dagger_1)
\end{bmatrix}
}{{Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) - {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2)}.
\end{equation*}
Therefore, 
\begin{equation*}
   \textrm{R.H.S. of Eq.~(\ref{eq:lem:rank2:unbias}) }  =   {
		    \begin{bmatrix}
{Q}^*(s,a^\dagger_1) & {Q}^*(s,a^\dagger_2)
\end{bmatrix}
(Q^\dagger)^{-1}
\begin{bmatrix}
{Q}^*(s^\dagger_1,a) \\
{Q}^*(s^\dagger_2,a)
\end{bmatrix}
}.
\end{equation*}
Let us now expand the above equation using the rank-2 assumption on $Q^*$. Denote by
\begin{align*}
F^\dagger \triangleq \begin{bmatrix}
f_1(s^\dagger_1) & f_2(s^\dagger_1)\\
f_1(s^\dagger_2) & f_2(s^\dagger_2)
\end{bmatrix}
\textrm{ and }
G^\dagger \triangleq \begin{bmatrix}
g_1(a^\dagger_1) & g_1(a^\dagger_2)\\
g_2(a^\dagger_1) & g_2(a^\dagger_2)
\end{bmatrix}.
% Q^\dagger = \underbrace{\begin{bmatrix}
% f_1(s^\dagger_1) & f_2(s^\dagger_1)\\
% f_1(s^\dagger_2) & f_2(s^\dagger_2)
% \end{bmatrix}}_{\triangleq F^\dagger}
% \underbrace{\begin{bmatrix}
% g_1(a^\dagger_1) & g_1(a^\dagger_2)\\
% g_2(a^\dagger_1) & g_2(a^\dagger_2)
% \end{bmatrix}}_{\triangleq G^\dagger}.
\end{align*}
Then, $Q^\dagger = F^\dagger G^\dagger$.
We claim that the matrices $F^\dagger$ and $G^\dagger$ are invertible. This is obvious because $\textrm{rank}(Q^\dagger)\leq \min\{\textrm{rank}(F^\dagger),\textrm{rank}(G^\dagger)\}$, which implies that $\textrm{rank}(F^\dagger) = \textrm{rank}(G^\dagger) = 2$. Therefore,
\begin{align*}
    \textrm{R.H.S. of Eq.~(\ref{eq:lem:rank2:unbias}) }  &= 
    \begin{bmatrix}
    f_1(s) & f_2(s)
    \end{bmatrix}G^\dagger(F^\dagger G^\dagger)^{-1}F^\dagger \begin{bmatrix}
    g_1(a)\\
    g_2(a)
    \end{bmatrix} \\
    & = \begin{bmatrix}
    f_1(s) & f_2(s)
    \end{bmatrix}G^\dagger (G^\dagger)^{-1}(F^\dagger)^{-1}F^\dagger \begin{bmatrix}
    g_1(a)\\
    g_2(a)
    \end{bmatrix}\\
    & =  \begin{bmatrix}
    f_1(s) & f_2(s)
    \end{bmatrix} \begin{bmatrix}
    g_1(a)\\
    g_2(a)
    \end{bmatrix}\\
    & = Q^*(s,a).
\end{align*}
This completes the proof of Lemma \ref{lem:rank2:unbiased}.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:rank2}]
 Since the context is clear, for simplicity, we omit the superscript $(t)$ for all the notation in the following proof. Denote by
\begin{align*}
    \hat{E} &\triangleq\hat{Q}(s^\dagger_1,a^\dagger_1)\hat{Q}(s^\dagger_2,a^\dagger_2) - \hat{Q}(s^\dagger_2,a^\dagger_1)\hat{Q}(s^\dagger_1,a^\dagger_2) \nonumber\\
    E^* &\triangleq {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) - {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2).
\end{align*}
We claim that 
\begin{equation}
\label{eq:rank2:prop:proof:E}
    |E^*|\geq \Delta V_{\min}^2\textrm{ and }|\hat{E}|\geq \Delta V_{\min}^2 
\end{equation}
To see this for $|E^*|$, we note that from Assumption \ref{assu:rank2_c}, $(1-c)^2{Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) - ((1+c)^2+\Delta) {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2)$. Therefore,
\begin{equation*}
    {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)\geq(1+\Delta){Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2)\geq {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2) + \Delta V_{\min}^2.
\end{equation*}
For $\hat{E}$, The condition in Proposition \ref{prop:rank2} implies that $Q^*(s,a)-\epsilon\hat{Q}(s,a)\leq Q^*(s,a)+\epsilon$. Since $Q^*(s,a)\geq V_{\min}$, we further obtain that $\big(1-\frac{\epsilon}{V_{\min}}\big) Q^*(s,a)  \leq \hat{Q}(s,a) \leq \big(1+\frac{\epsilon}{V_{\min}}\big)Q^*(s,a)$. Note that $\epsilon$ is assumed to be $\epsilon\leq cV_{\min}$. Hence,
\begin{equation*}
    (1-c) Q^*(s,a)  \leq \hat{Q}(s,a) \leq (1+c)Q^*(s,a)
\end{equation*}
Apply the above inequality and Assumption \ref{assu:rank2_c},
\begin{align*}
    \hat{E}&\geq (1-c)^2{Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) - (1+c)^2 {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2)\\
    &\geq \Delta {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2)\\
    &\geq \Delta V_{\min}^2.
\end{align*}
Let us first expand out the estimator $\bar{Q}^{(t)}$.
\begin{align}
    \bar{Q}(s,a) = & \frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a)}{\hat{E}}-\frac{\hat{Q}(s,a_2^\dagger)\hat{Q}(s_2^\dagger,a_1^\dagger)\hat{Q}(s_1^\dagger,a)}{\hat{E}}\nonumber\\
    &-\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_1^\dagger,a_2^\dagger)\hat{Q}(s_2^\dagger,a)}{\hat{E}}+\frac{\hat{Q}(s,a_2^\dagger)\hat{Q}(s_1^\dagger,a_1^\dagger)\hat{Q}(s_2^\dagger,a)}{\hat{E}}.
\end{align}
Similarly, by applying Lemma \ref{lem:rank2:unbiased}, we have
\begin{align}
    {Q}^*(s,a) = & \frac{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)}{{E}^*}-\frac{{Q}^*(s,a_2^\dagger){Q}^*(s_2^\dagger,a_1^\dagger){Q}^*(s_1^\dagger,a)}{{E}^*}\nonumber\\
    &-\frac{{Q}^*(s,a_1^\dagger){Q}^*(s_1^\dagger,a_2^\dagger){Q}^*(s_2^\dagger,a)}{{E}^*}+\frac{{Q}^*(s,a_2^\dagger){Q}^*(s_1^\dagger,a_1^\dagger){Q}^*(s_2^\dagger,a)}{{E}^*}.
\end{align}
Therefore, by triangle inequality
\begin{align}
    |\bar{Q}(s,a)-Q^*(s,a)|\leq \bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a)}{\hat{E}} -  \frac{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)}{{E}^*}\bigg|\nonumber\\
    + \bigg|\frac{\hat{Q}(s,a_2^\dagger)\hat{Q}(s_2^\dagger,a_1^\dagger)\hat{Q}(s_1^\dagger,a)}{\hat{E}}-\frac{{Q}^*(s,a_2^\dagger){Q}^*(s_2^\dagger,a_1^\dagger){Q}^*(s_1^\dagger,a)}{{E}^*}\bigg|\nonumber\\
    + \bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_1^\dagger,a_2^\dagger)\hat{Q}(s_2^\dagger,a)}{\hat{E}}-\frac{{Q}^*(s,a_1^\dagger){Q}^*(s_1^\dagger,a_2^\dagger){Q}^*(s_2^\dagger,a)}{{E}^*}\bigg|\nonumber\\
    + \bigg|\frac{\hat{Q}(s,a_2^\dagger)\hat{Q}(s_1^\dagger,a_1^\dagger)\hat{Q}(s_2^\dagger,a)}{\hat{E}}-\frac{{Q}^*(s,a_2^\dagger){Q}^*(s_1^\dagger,a_1^\dagger){Q}^*(s_2^\dagger,a)}{{E}^*}\bigg| \label{eq:rank2:prop:proof:difference}
\end{align}
We remark that the four terms in the R.H.S. of Eq.~(\ref{eq:rank2:prop:proof:difference}) can be bounded by essentially the same steps. Below, we derive upper bound  on the first term.
\begin{align}
    &\bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a)}{\hat{E}} -  \frac{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)}{{E}^*}\bigg|\nonumber\\
    & = \bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a)E^*- {Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)\hat{E}}{\hat{E}E^*}\bigg|\nonumber\\
    & = \bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a)\big( {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) - {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2)\big)}{\hat{E}E^*}-\nonumber\\
    &\quad\:\:\frac{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)\big(\hat{Q}(s^\dagger_1,a^\dagger_1)\hat{Q}(s^\dagger_2,a^\dagger_2) - \hat{Q}(s^\dagger_2,a^\dagger_1)\hat{Q}(s^\dagger_1,a^\dagger_2)\big)}{\hat{E}E^*} \bigg|\nonumber\\
    &\leq \underbrace{\bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) -{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)\hat{Q}(s^\dagger_1,a^\dagger_1)\hat{Q}(s^\dagger_2,a^\dagger_2) }}{\hat{E}E^*}\bigg|}_{=: A}\nonumber\\
    & + \underbrace{\bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_2,a^\dagger_1){Q}^*(s^\dagger_1,a^\dagger_2) - {{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a) \hat{Q}(s^\dagger_2,a^\dagger_1)\hat{Q}(s^\dagger_1,a^\dagger_2)}}{\hat{E}E^*}\bigg|}_{=: B}, \label{eq:rank2:prop:proof:AB}
\end{align}
where the last inequality follows from triangle inequality. Let us now upper bound the terms $A$ and $B$ in Eq.~(\ref{eq:rank2:prop:proof:AB}). We start with term $A$ below. By triangle inequality, we have that
\begin{align}
    A &\leq \frac{1}{|\hat{E}E^*|}\bigg(\Big|{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) -{Q}^*(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)}\Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) -{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)}\Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) -{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)}\Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) -{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a) \hat{Q}(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)}\Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a) \hat{Q}(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2) -{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)\hat{Q}(s^\dagger_1,a^\dagger_1)\hat{Q}(s^\dagger_2,a^\dagger_2) }}\Big| \bigg) \nonumber\\
    &= \frac{1}{|\hat{E}E^*|}\bigg(\Big|{\hat{Q}(s,a_1^\dagger)-Q^*(s,a_1^\dagger)\Big|\Big|\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)} \Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger)\Big|\Big|\hat{Q}(s_2^\dagger,a_2^\dagger)-{Q}^*(s_2^\dagger,a_2^\dagger)\Big|\Big|\hat{Q}(s_1^\dagger,a) {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)}\Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger)\Big|\Big|\hat{Q}(s_1^\dagger,a) - {Q}^*(s_1^\dagger,a)\Big|\Big| {Q}^*(s^\dagger_1,a^\dagger_1){Q}^*(s^\dagger_2,a^\dagger_2)}\Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a) \Big|\Big|{Q}^*(s^\dagger_1,a^\dagger_1)-\hat{Q}(s^\dagger_1,a^\dagger_1)\Big|{Q}^*(s^\dagger_2,a^\dagger_2)}\Big| \nonumber\\
    &+\Big|{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a) \hat{Q}(s^\dagger_1,a^\dagger_1)\Big|\Big|{Q}^*(s^\dagger_2,a^\dagger_2)-\hat{Q}(s^\dagger_2,a^\dagger_2)}\Big| \bigg) \nonumber\\
    &\leq \frac{5V_{\max}^4}{\Delta^2 V_{\min}^4}\cdot \epsilon,
\end{align}
where the last inequality follows from our bounds on $\hat{E}$ and $E^*$ (cf. Eq.~(\ref{eq:rank2:prop:proof:E})) and the facts that $|\hat{Q}(s,a)|\leq V_{\max}$, $|Q^*(s,a)|\leq V_{\max}$ and $\hat{Q}(s,a)-Q^*(s,a)|\leq \epsilon$. Following the same step, one can also obtain the same bound for the term $B$ in Eq.~(\ref{eq:rank2:prop:proof:AB}): $B\leq \frac{5V_{\max}^4}{\Delta^2 V_{\min}^4}\cdot \epsilon$. To summarize, we have the following bound for the first term on the R.H.S. of Eq.~(\ref{eq:rank2:prop:proof:difference}):
\begin{equation*}
    \bigg|\frac{\hat{Q}(s,a_1^\dagger)\hat{Q}(s_2^\dagger,a_2^\dagger)\hat{Q}(s_1^\dagger,a)}{\hat{E}} -  \frac{{Q}^*(s,a_1^\dagger){Q}^*(s_2^\dagger,a_2^\dagger){Q}^*(s_1^\dagger,a)}{{E}^*}\bigg|\leq  \frac{10V_{\max}^4}{\Delta^2 V_{\min}^4}\cdot \epsilon.
\end{equation*}
It is easy to see that the same reasoning can be applied to bound each of the remaining three terms on the R.H.S. of Eq.~(\ref{eq:rank2:prop:proof:difference}) and obtain the same upper bound $\frac{10V_{\max}^4}{\Delta^2 V_{\min}^4}\cdot \epsilon$. Therefore, we finally arrive at the conclusion that
\begin{equation*}
    |\bar{Q}(s,a)-Q^*(s,a)|\leq \frac{40V_{\max}^4}{\Delta^2 V_{\min}^4}\cdot \epsilon = \frac{40R_{\max}^4}{\Delta^2 R_{\min}^4}\cdot \epsilon.
\end{equation*}
\end{proof}

==> rankr.tex <==
\section{Rank-$r$ Reinforcement Learning}
\label{sec:rankr}


Based on the intuition developed in Section \ref{sec:rank1}, we consider a more general rank-$r$ setup. For notational convenience,
given $Q: \mS \times \mA \to \RR$ and $\mS' \subset \mS, \mA' \subset \mA$, we let $Q(\mS', \mA')$ denote the $|\mS'| \times |\mA'|$ matrix $\big[ Q(s,a): ~(s,a) \in \mS' \times \mA' \big]$, whose entries are indexed by $(s,a) \in \mS' \times \mA'$. When $\mS' = \{ s \}$, we write $Q(s, \mA') = Q(\{s\}, \mA' )$ with abuse of notation. Given $M \in \RR^{m \times n}$, we let $M^{\dagger} \in \RR^{n \times m}$ denote the Moore-Penrose pseudoinverse of $M$.

The central idea is the same as before: although $Q^*(\mS^{(t)},\mA^{(t)})\in\mathbb{R}^{n\times m}$ is an array of $nm$ real numbers, it has only $r (n+m-r)$ degrees of freedom with $r$-dimensional column and row spaces, when $\textrm{rank}(Q^*(\mS^{(t)},\mA^{(t)})) = r \leq \min\{ m, n \}$; as a result, one can successfully restore $Q^*(\mS^{(t)},\mA^{(t)})$ by exploring only $r$ entire rows and columns. There is, however, a small caveat that the $r$ rows and $r$ should be carefully chosen so that they are not degenerate, i.e., the $r$ rows span the entire row space of $Q^*(\mS^{(t)},\mA^{(t)})$ (the $r$ columns span the entire column space of $Q^*(\mS^{(t)},\mA^{(t)})$, respectively). Towards this end, we first define the notion of anchor states and actions.



\begin{defn}\label{defn:anchor_set}
(Anchor States and Actions) 
A set of states $\mS^{\sharp} = \{s^\sharp_i\}_{i=1}^{R_s} \subset \mS$ and actions $\mA^{\sharp} = \{a^\sharp_i\}_{i=1}^{R_a} \subset\mA$ for some $R_s, R_a$ are called anchor states and actions for $Q^*$ if $\textrm{rank}~ Q^*(\mS^{\sharp}, \mA^{\sharp} ) = r$.
\end{defn}

That is, there are $r$ states in the anchor states $\mS^\sharp$ such that their corresponding performance, $Q^*(s,\mA^\sharp)$, on the anchor actions $\mA^\sharp$ are linearly independent. In other words, $\mS^\sharp$ are states with diverse performance on actions $\mA^\sharp$. Likewise, similar interpretation holds for $\mA^\sharp$ if we look at the columns of $ Q^*(\mS^{\sharp}, \mA^{\sharp} )$. Overall, anchor states/actions are intuitively sets of sufficiently diverse states/actions whose performance capture different aspects of the task reflected on $Q^*$. 

% (another version) That is, for any $s \in \mS$, $Q^*(s, \mA)$ can be expressed as a linear combination of the rows of $Q^*(\mS^{\sharp}, \mA)$ and likewise, $Q^*(\mS, a)$ can be expressed as a linear combination of the columns of $Q^*(\mS, \mA^{\sharp})$. Intuitively, $\mS^\sharp$ is a set of `representative' states that contain information about $Q^*(\mS,\mA)$; a similar interpretation is possible for $\mA^\sharp$. In other words, anchor states/actions are sets of sufficiently diverse states/actions whose performance capture different aspects of the task reflected on $Q^*$. 

% for any $s \in \mS$, $Q^*(s, \mA)$ can be expressed as a linear combination of the rows of $Q^*(\mS^{\sharp}, \mA)$ and likewise, $Q^*(\mS, a)$ can be expressed as a linear combination of the columns of $Q^*(\mS, \mA^{\sharp})$. Intuitively, $\mS^\sharp$ is a set of `representative' states that contain information about $Q^*(\mS,\mA)$; a similar interpretation is possible for $\mA^\sharp$. 

% In other words, anchor states/actions are sets of sufficiently diverse states/actions whose performance capture different aspects of the task reflected on $Q^*$. 

%\red{DG: I think the paragraph below should go to introduction or somewhere else?}
Indeed, $\mS^{\sharp}$ and $\mA^{\sharp}$ will be applied to construct our exploration set and we want them to have small size. Finding only few diverse states and actions are arguably easy in practical task --- indeed, for several stochastic control tasks experimented in Section~\ref{sec:empirical}, we simply pick few states and actions that are far from each other in the respective space. We remark that assuming some "anchor" elements (i.e., elements having some special, relevant properties) are common in feature-based reinforcement learning~\cite{yang2019sample,duan2019state} or matrix factorization such as topic modeling~\cite{arora2012learning}.

% Based on the intuition developed in Section \ref{sec:rank1}, we consider a more general rank-$r$ setup. The central idea is the same as before: although $Q^* \in \RR^{m \times n}$ is an array of $mn$ real numbers, it has only $r (m+n-r)$ degrees of freedom when $\textrm{rank}(Q^*) = r \leq \min\{ m, n \}$; as a result, one can successfully restore $Q^*$ by exploring only $r$ rows and columns. There is, however, a small caveat that the $r$ rows and $r$ should be carefully chosen so that they are not degenerate, i.e., the $r$ rows span the entire row space of $Q^*$ (the $r$ columns span the entire column space of $Q^*$, respectively). Towards this end, we first define the notion of anchor states and actions.

% For $Q: \mS \times \mA \to \RR$ and $\mS' \subset \mS, \mA' \subset \mA$, we let $Q(\mS', \mA')$ denote the $|\mS'| \times |\mA'|$ matrix $\big[ Q(s,a): ~(s,a) \in \mS' \times \mA' \big]$, whose entries are indexed by $(s,a) \in \mS' \times \mA'$. When $\mS' = \{ s \}$, we write $Q(s, \mA') = Q(\{s\}, \mA' )$ with abuse of notation. Given $M \in \RR^{m \times n}$, we let $M^{\dagger} \in \RR^{n \times m}$ denote the Moore-Penrose pseudoinverse of $M$.

% \begin{defn}
% (Anchor States and Actions) 
% Let $r = \textrm{rank}~ Q^*(\mS, \mA)$. A set of states $\mS^{\sharp} = \{s^\sharp_i\}_{i=1}^{R_s} \subset \mS$ and actions $\mA^{\sharp} = \{a^\sharp_i\}_{i=1}^{R_a} \subset\mA$ for some $R_s, R_a$ are called anchor states and actions if $\textrm{rank}~ Q^*(\mS^{\sharp}, \mA^{\sharp} ) = r$.
% \end{defn}

% That is, for any $s \in \mS$, $Q^*(s, \mA)$ can be expressed as a linear combination of the rows of $Q^*(\mS^{\sharp}, \mA)$ and likewise, $Q^*(\mS, a)$ can be expressed as a linear combination of the columns of $Q^*(\mS, \mA^{\sharp})$. Intuitively, $\mS^\sharp$ is a set of `representative' states that contain information about $Q^*(\mS,\mA)$; a similar interpretation is possible for $\mA^\sharp$. In other words, anchor states/actions are sets of sufficiently diverse states/actions whose performance capture different aspects of the task reflected on $Q^*$. 

% %\red{DG: I think the paragraph below should go to introduction or somewhere else?}
% Indeed, $\mS^{\sharp}$ and $\mA^{\sharp}$ will be our exploration set and we want them to have small size. Finding only few such states and actions are arguably easy in practical task --- indeed, for several stochastic control tasks experimented in Section~\ref{sec:empirical}, we simply pick few states and actions that are far from each either in the respective space. We remark that assuming some "anchor" elements (i.e., elements having some special, relevant properties) are common in feature-based reinforcement learning~\cite{yang2019sample,duan2019state} or matrix factorization such as topic modeling~\cite{arora2012learning}.


{\bf Algorithmic Choices Developed} We are now ready to describe our exploration and ME strategies which amount to exploring the entire rows corresponding to anchor states and the columns corresponding to anchor actions. At initialization (i.e., $t=0$), we select a set of anchor states $\mS^{\sharp} \subset \mS$ and a set of anchor actions $\mA^{\sharp} \subset \mA$, and fix $\mS^{\sharp}, \mA^{\sharp}$ through all $T$ iterations. Then, at each $t=1,\dots, T$:
\begin{itemize}
   % \item Choice of anchor states/actions: pick a set of anchor states $\mS^{\sharp} \subset \mS$ and a set of anchor actions $\mA^{\sharp} \subset \mA$. It is possible to do this only once at the beginning and fix $\mS^{\sharp}, \mA^{\sharp}$ through all $T$ iterations.
    \item Discretization: After obtaining the $\beta^{(t)}$-nets $\mS^{(t)}$ and $\mA^{(t)}$, augment them with the anchor states and actions: $\bar{\mS}^{(t)}\gets \mS^{(t)}\cup \mS^{\sharp}$ and $\bar{\mA}^{(t)}\gets \mA^{(t)}\cup \mA^{\sharp}$.
    \item
    Choice of exploration set $\Omega^{(t)}$:
    %At each $t =1, \ldots, T$, 
    %choose an anchor state $s^{\dagger} \in \mS^{(t)}$ and an anchor action $a^{\dagger} \in \mA^{(t)}$. 
    %Then 
    Let $\Omega^{(t)} = \{ (s,a) \in \bar{\mS}^{(t)} \times \bar{\mA}^{(t)}: s \in \mS^{\sharp} \text{ or } a \in \mA^{\sharp} \}$.
    
    \item
    Matrix Estimation subroutine: For $(s,a) \in \mS^{(t)} \times \mA^{(t)}$, let
    \begin{equation}\label{eqn:ME_rankr}
        \bar{Q}^{(t)}(s,a) = \hat{Q}^{(t)} (s, \mA^{\sharp} ) \big[ \hat{Q}^{(t)}(\mS^{\sharp}, \mA^{\sharp} ) \big]^{\dagger} \hat{Q}^{(t)}(\mS^{\sharp}, a )
    \end{equation}
    where $\big[ \hat{Q}^{(t)}(\mS^{\sharp}, \mA^{\sharp} ) \big]^{\dagger}$ is the Moore-Penrose pseudoinverse of $\hat{Q}^{(t)}(\mS^{\sharp}, \mA^{\sharp} )$.
\end{itemize}
% Rule to choose $\beta^{(t)}$
% Rule to choose $N^{(t)}$
% For simplicity, we may assume $R_s = | \mS^{\sharp} | = r$ and $R_a = |\mA^{\sharp}| = r$.
% We note that the size of the exploration set is much smaller than the cardinality of the entire (discretized) state-action space at iteration $t$, 
% i.e., $|\Omega^{(t)}| = r \big( |\mS^{(t)}| + |\mA^{(t)}| - r \big) \ll | \mS^{(t)} | |\mA^{(t)}|$. 




For the convenience of analysis, we may assume $\mS^{(t)} \cap \mS^{\sharp} = \mA^{(t)} \cap \mA^{\sharp} = \emptyset$.
Moreover, we note here that if $R_s = | \mS^{\sharp} | = r$ and $R_a = |\mA^{\sharp}| = r$ (or in general, a constant mulitple of $r$), then the size of the exploration set is much smaller than the cardinality of 
the entire (discretized) state-action space at iteration $t$, i.e., $|\Omega^{(t)}| = r \big( |\mS^{(t)}| + |\mA^{(t)}| +r \big) \ll | \mS^{(t)} | |\mA^{(t)}|$. \red{For simplicity, let $|\mS^{\sharp}| = |\mA^{\sharp}| = r$.}




{\bf Theoretical Guarantees} We have the following guarantee for the Matrix Estimation subroutine. For a matrix $X$, denote by $\sigma_i(X)$ its $i$-th singular value, and assume that the singular values are arranged in descending order, i.e., $ \sigma_1(X) \geq \sigma_2(X)\geq\dots\geq\sigma_n(X)$.
\begin{prop}\label{prop:rankr_simplified}[Simplified version of Proposition \ref{prop:rankr}]
    Let $\Omega^{(t)}$ and $\bar{Q}^{(t)}$ as described above and let $|\mS^{\sharp}| = |\mA^{\sharp}| = r$.
    For any $\epsilon \leq \frac{1}{2r} \sigma_r\big( Q^*(\mS^{\sharp}, \mA^{\sharp} ) \big)$, if $\max_{(s,a) \in \Omega^{(t)}} \big| \hat{Q}^{(t)}(s,a) - Q^*(s,a) \big| \leq \epsilon$, then
    \begin{align*}
        \max_{(s,a) \in \mS^{(t)}\times \mA^{(t)}} \big| \bar{Q}^{(t)}(s,a) - Q^*(s,a) \big|		\leq c(r; \mS^{\sharp}, \mA^{\sharp} ) \epsilon
    \end{align*}
    where $c(r; \mS^{\sharp}, \mA^{\sharp} ) = \Big( 6\sqrt{2} \big( \frac{r}{\sigma_r ( Q^*(\mS^{\sharp}, \mA^{\sharp} ))} \big) + 2(1+\sqrt{5}) \big( \frac{r}{\sigma_r ( Q^*(\mS^{\sharp}, \mA^{\sharp} ))} \big)^2 \Big) V_{\max}$.
\end{prop}

With Proposition \ref{prop:rankr_simplified} at hand, we can obtain the following theorem as a Corollary of Theorem \ref{thm:generic} for the rank-$r$ setup. The proof basically remains the same, and we only need to additionally verify $\max_{(s,a) \in \Omega^{(t)}} \big| \hat{Q}^{(t)}(s,a) - Q^*(s,a) \big| \leq \frac{1}{2r} \sigma_r\big( Q^*(\mS^{\sharp}, \mA^{\sharp} ) \big)$ for all $t$ to use Proposition \ref{prop:rankr_simplified}.


\begin{thm}
\label{thm:rankr}
    % Let there be a rank-1 MDP problem such that (i) $R(s,a) \in [R_{\min}, R_{\max}]$ for all $(s,a) \in \mS \times \mA$ where $R_{\min} > 0$ and (ii) $\gamma < \frac{R_{\min}}{14 R_{\max}}$. 
    % Suppose that we run Algorithm \ref{alg:generic} initialized at $Q^{(0)} \equiv 0$ to solve the MDP problem with the exploration and the matrix estimation steps as described above.
    
    Consider the rank-$r$ setting in this section. Suppose that we run  Algorithm \ref{alg:generic} with the exploration and the matrix estimation steps as described.
    If $\gamma \leq \frac{1}{2 c(r; \mS^{\sharp}, \mA^{\sharp} )}$, then the following holds.
    \begin{enumerate}
    \item
    For any $\delta > 0$, we have 
    \begin{equation*}%\label{eqn:geom_rate}
        \sup_{ (s,a) \in \mS \times \mA } \big| Q^{(t)}(s,a) - Q^*(s,a) \big|
            \leq \big(  2 c(r; \mS^{\sharp}, \mA^{\sharp} ) \gamma  \big)^t V_{\max},
             \quad\textrm{for all } t = 1, \ldots, T
    \end{equation*}
    with probability at least $1 - \delta$ by choosing algorithmic parameters $\beta^{(t)}, N^{(t)}$ appropriately.
    % $\beta^{(t)} = \frac{V_{\max}}{8L} \big( \frac{14 R_{\max}}{R_{\min}} \gamma \big)^t$, $N^{(t)} = 8 \big( \frac{14 R_{\max}}{R_{\min}} \gamma \big)^{-2(t-1)} \log\big(\frac{2 | \Omega^{(t)} | T}{\delta}\big)$ for $t = 1, \ldots, T$.
    
    \item
    For any $\epsilon > 0$ and $\delta > 0$, it suffices to set $T = \Theta( \log \frac{1}{\epsilon} )$ and use $\tilde{O}( \frac{1}{\epsilon^{d+2}} \cdot \log \frac{1}{\delta} )$ samples to achieve $\sup_{(s,a) \in \mS \times \mA} \big| Q^{(T)}(s,a) - Q^*(s,a) \big| \leq \epsilon$ with probability at least $1 - \delta$.
    \end{enumerate}
\end{thm}



\red{DG: TODO -- add remarks/discussion
\begin{itemize}
    \item 
    approx rank-r
    \item
    why we couldn't use existing ME methods
    \item
    limited range of $\gamma$
\end{itemize}
}


{\bf Approximate Rank-$r$ Reinforcement Learning (Appendix \ref{sec:app_r})}: \red{Left for Dogyoon} due to space limit, xxx, descirbe the setting and results informally. with a corresponind anchor states and actions for the approxiamte rank r case, suppose we run the rank-r algorithms.


\begin{rem}
{\bf Why existing ME methods are insufficient technically} Beyond the scarcity of 
%As mentioned, although ME is a relatively mature field, 
$\ell_\infty$ guarantees in literature,
%remains a difficult task with very sparse results. 
%Beyond the adaptive feature that allows us to develop a suitable ME method, 
%We remark that indeed 
there is indeed a deeper technical reason that justifies 
%makes existing methods insufficient and hence 
the necessity of our new development. Traditional ME considers the static problem: given a single true matrix $X$ and some noisy entries, recover $X$. To get any guarantee, 
majority of literature requires the $\mu$-incoherence assumption(citation), which roughly requires both the left and right singular vectors of $X$ to be not sparse. 
%This assumption works fine for the static case. 
However, in our problem, the $|\mS^{(t)}|\times |\mA^{(t)}|$ matrix we want to estimate at each iteration comes from a \emph{common} source: it is the $Q^*$-function restricted to our discretized set. To apply traditional techniques, we would assume that for \emph{every} iteration, for the scale we choose, we can always find a discretization so that the resulting matrix is $\mu$-incoherent. This is an extremely strong technical assumption, whose operational meaning is also unclear. In contrast, our new development has a much more reasonable and interpretable condition, which also leads to a simpler proof. %Nevertheless, existing ME methods often work well in practice and we will also compare with them in our experiments. 
How to devise new proof technique to obtain guarantees for existing methods is an valuable open question.  
\end{rem}

\begin{rem}
{\bf  Potential Improvements}
%Our generic Theorem \ref{thm:generic} and the rank-$r$ results above demonstrates the value of our low-rank framework for efficient RL. 
While it requires certain condition on $\gamma$, as a first attempt, our new development can serve as a starting point for improvement. To obtian a wider range of $\gamma$, it is by now clear that there are two potential sources: obtaining better estimates when we explore a $(s,a)\in\Omega^{(t)}$ or proving sharp bounds (better $c_\eta$) for ME. For the first, one may try to do multi-step lookaheads. However, extra care must be paid due to the continuous action space if only finitely-many actions are tried. For the second, designing new ME methods are valuable in bridging the gap between ME literature and RL. Such methods should, however, be appropriate and meaningful in the RL context.
We believe both are important and fruitful inquires for efficient RL.
\end{rem}



% We generalize rank-$1$ to rank-$r$ case using the intuition developed. In the previous section, we are motivated to explore an entire column and row so as to understand the one-dimensional "column space" and "row space". Naturally, we extend our success to explore $r$ entire columns and $r$ entire rows when $Q^*$ is rank-$r$. There is, however, a small complication.
% Rank-$1$ scenario is special in the sense that exploring any row and column suffices as the spaces are only one- dimensional. For rank-$r$ $Q^*$, we need to be smarter about the $r$ rows and $r$ columns so that they do not result in degenerated case. Towards this end, we first define the following notion of anchor states and actions.
% \begin{defn}
% (Anchor States and Actions) A set of $r$ states $\{s^\dagger_i\}_{i=1}^r\subset \mS$ and $r$ actions $\{a^\dagger_i\}_{i=1}^r\subset\mA$ are called anchor states and actions if the $r\times r$ matrix $\mathbb{Q}^\dagger$, whose $ij$-th entry equals to $Q^*(s_i^\dagger,a_j^\dagger)$, is non-singular.
% \end{defn}
% We suppose that we have access to a set of anchor states $\{s^\dagger_i\}_{i=1}^r\subset \mS$ and anchor actions $\{a^\dagger_i\}_{i=1}^r\subset\mA$. To provide some justification, beyond being a technical condition, anchor states and actions are indeed operationally meaningful as we now illustrate. For example, consider $r=2$. Non-singular $\mathbb{Q}^\dagger$ is equivalent to $\textrm{det}(\mathbb{Q}^\dagger)=Q^*(s_1^\dagger,a_1^\dagger)Q^*(s_2^\dagger,a_2^\dagger)-Q^*(s_1^\dagger,a_2^\dagger)Q^*(s_2^\dagger,a_1^\dagger)>0$. Suppose $Q^*$ is positive, then the condition means that we find two states ($s_1^\dagger,s_2^\dagger$) and two actions ($a_1^\dagger,a_2^\dagger$) such that $a^\dagger_1$ is better than $a^\dagger_2$ for $s_1^\dagger$ and $a^\dagger_2$ is better than $a^\dagger_1$ for $s_2^\dagger$. These can be readily available. For general $r$, non-singular $\mathbb{Q}^\dagger$ means that if we look at rows, say the $i$-th row $[Q^*(s_i^\dagger,a_1^\dagger),\dots,Q^*(s_i^\dagger,a_r^\dagger)]$, then it is not a linear combination of other rows, i.e., the performance of these actions varies to a certain degree for the anchor states; similar interpretation can be obtained if we look at columns. Overall, anchor states and actions are intuitively different states and actions of the space whose performance varies in the task and that capture different aspects of the task. 
% %in terms of the tasks rather than just the raw value of stats and actions.
% Finding only few such states and actions are arguably easy in practical task --- indeed, for several stochastic control tasks experimented in Section~\ref{sec:empirical}, we simply pick few states and actions that are far from each either in the respective space. We remark that assuming some "anchor" elements (i.e., elements having some special, relevant properties) are common in feature-based reinforcement learning~\cite{yang2019sample,duan2019state} or matrix factorization such as topic modeling~\cite{arora2012learning}.
% %i.e., states and actions that capture different aspects of the task. 

% {\bf Algorithmic Choices Developed} We are now ready to describe our exploration and ME strategies which amount to exploring the entire $r$ rows corresponding to anchor states and the entire $r$ columns corresponding to anchor actions. At each $t=1,\dots, T$:
% \begin{itemize}
%     \item Discretization: After obtaining the $\beta^{(t)}$-nets $\mS^{(t)}$ and $\mA^{(t)}$, augment them with the anchor states and actions: $\mS^{(t)}\gets \mS^{(t)}\cup\{s^\dagger_i\}_{i=1}^r$ and   $\mA^{(t)}\gets \mA^{(t)}\cup\{a^\dagger_i\}_{i=1}^r$
%     \item
%     Choice of exploration set $\Omega^{(t)}$:
%     %At each $t =1, \ldots, T$, 
%     %choose an anchor state $s^{\dagger} \in \mS^{(t)}$ and an anchor action $a^{\dagger} \in \mA^{(t)}$. 
%     %Then 
%     Let $\Omega^{(t)} = \{ (s,a) \in \mS^{(t)} \times \mA^{(t)}: s \in \{s^{\dagger}_i\}_{i=1}^r \text{ or } a \in \{a^{\dagger}_i\}_{i=1}^r \}$.
    
%     \item
%     Matrix Estimation subroutine: Denote by $\hat{\mathbb{Q}}^{(t),\dagger}$ the $r\times r$ matrix whose $ij$-th entry equals to $\hat{Q}^{(t)}(s_i^\dagger,a_j^\dagger)$. 
%     For $(s,a) \in \mS^{(t)} \times \mA^{(t)}$, we let
%     	\begin{equation*}
% 		    \bar{Q}^{(t)}(s,a) = {
% 		    \begin{bmatrix}
% \hat{Q}^{(t)}(s,a^\dagger_1) & \hat{Q}^{(t)}(s,a^\dagger_2) &\cdots &\hat{Q}^{(t)}(s,a^\dagger_r)
% \end{bmatrix}
% \big(\hat{\mathbb{Q}}^{(t),\dagger}\big)^{-1}
% % \begin{bmatrix}
% % \hat{Q}^{(t)}(s_2^\dagger,a^\dagger_2) & -\hat{Q}^{(t)}(s^\dagger_1,a^\dagger_2)\\
% % -\hat{Q}^{(t)}(s^\dagger_2,a^\dagger_1) & \hat{Q}^{(t)}(s^\dagger_1,a^\dagger_1)
% % \end{bmatrix}
% \begin{bmatrix}
% \hat{Q}^{(t)}(s^\dagger_1,a) \\
% \hat{Q}^{(t)}(s^\dagger_2,a)\\
% \vdots\\
% \hat{Q}^{(t)}(s^\dagger_r,a)

% \end{bmatrix}
% }
% 		\end{equation*}
		
    
% \end{itemize}
% % Rule to choose $\beta^{(t)}$
% % Rule to choose $N^{(t)}$
% Again, note that $|\Omega^{(t)}| = r|\mS^{(t)}| + r|\mA^{(t)}| - r^2$, which is much smaller than $ | \mS^{(t)} | |\mA^{(t)}|$, the cardinality of the entire (discretized) state-action space at iteration $t$. 

% {\bf Theoretical Guarantees}
% For a $n\times n$ matrix $X$, we denote by $\sigma_i(X)$ its $i$-th singular value and let $\sigma_{\min}(X) \triangleq\min_{i\in[n]}\sigma_i(X)$. 
% \red{Left for Dogyoon}

% {\bf Approximate Rank-$r$ Reinforcement Learning (Appendix \ref{sec:app_r})}: due to space limit, xxx, descirbe the setting and results informally. with a corresponind anchor states and actions for the approxiamte rank r case, suppose we run the rank-r algorithms.


% \begin{rem}
% {\bf Why existing ME methods are insufficient technically} Beyond the scarcity of 
% %As mentioned, although ME is a relatively mature field, 
% $\ell_\infty$ guarantees in literature,
% %remains a difficult task with very sparse results. 
% %Beyond the adaptive feature that allows us to develop a suitable ME method, 
% %We remark that indeed 
% there is indeed a deeper technical reason that justifies 
% %makes existing methods insufficient and hence 
% the necessity of our new development. Traditional ME considers the static problem: given a single true matrix $X$ and some noisy entries, recover $X$. To get any guarantee, 
% majority of literature requires the $\mu$-incoherence assumption(citation), which roughly requires both the left and right singular vectors of $X$ to be not sparse. 
% %This assumption works fine for the static case. 
% However, in our problem, the $|\mS^{(t)}|\times |\mA^{(t)}|$ matrix we want to estimate at each iteration comes from a \emph{common} source: it is the $Q^*$-function restricted to our discretized set. To apply traditional techniques, we would assume that for \emph{every} iteration, for the scale we choose, we can always find a discretization so that the resulting matrix is $\mu$-incoherent. This is an extremely strong technical assumption, whose operational meaning is also unclear. In contrast, our new development has a much more reasonable and interpretable condition, which also leads to a simpler proof. %Nevertheless, existing ME methods often work well in practice and we will also compare with them in our experiments. 
% How to devise new proof technique to obtain guarantees for existing methods is an valuable open question.  
% \end{rem}

% \begin{rem}
% {\bf  Potential Improvements}
% Our generic Theorem \ref{thm:generic} and the rank-$r$ results above provides the first We believe that our new development can serve as a starting point
% \end{rem}




% -------------------------------------------

% With the generic results at hand, we now provide explicit sampling scheme for selecting the subset $\Omega^{(t)}$  and the corresponding algorithms for the matrix estimation oracle. The main goal is to demonstrate a practical and provable oracle that satisfying the desired performance guarantees, i.e., Assumption \ref{assu:me}, under proper conditions. To develop the intuition and facilitate a better understanding, let us start with the rank-1 case.

% Throughout this section, we consider reinforcement learning when $Q^*$ is rank-1. That is, there exist some functions $f:\mS\rightarrow \mathbb{R}$ and $g:\mA\rightarrow\mathbb{R}$ such that 
% \begin{equation*}
%     Q^*(s,a) = \sum_{i=1}^rf_i(s)\cdot g_i(a).
% \end{equation*}
% In Section \ref{subsec:rank1_alg}, we first provide intuitions for developing a suitable matrix estimation oracle under this setting and then introduce the full algorithm. Provable guarantees are given in Section \ref{subsec:rank1_theory}.



% \subsection{Algorithm}
% \label{subsec:rank2_alg}
% {\bf Notation.} For convenience, we define the following matrix notation. Fix an iteration $t$, denote by
% \begin{equation*}
%     \hat{\mathbb{Q}}^{(t),\dagger} = \begin{bmatrix}
% \hat{Q}^{(t)}(s_1^\dagger,a^\dagger_1) & \hat{Q}^{(t)}(s^\dagger_1,a^\dagger_2) & \cdots & \hat{Q}^{(t)}(s^\dagger_1, a^\dagger_r)\\
% \hat{Q}^{(t)}(s_2^\dagger,a^\dagger_1) & \hat{Q}^{(t)}(s^\dagger_2,a^\dagger_2) & \cdots & \hat{Q}^{(t)}(s^\dagger_2, a^\dagger_r)\\
% \vdots & \vdots & \vdots & \vdots\\
% \hat{Q}^{(t)}(s_r^\dagger,a^\dagger_1) & \hat{Q}^{(t)}(s^\dagger_r,a^\dagger_2) & \cdots & \hat{Q}^{(t)}(s^\dagger_r, a^\dagger_r)
% \end{bmatrix}
%     \mathbb{Q}^{\dagger} = \begin{bmatrix}
% {Q}^*(s_1^\dagger,a^\dagger_1) & {Q}^{*}(s^\dagger_1,a^\dagger_2) & \cdots & {Q}^{*}(s^\dagger_1, a^\dagger_r)\\
% {Q}^*(s_2^\dagger,a^\dagger_1) & {Q}^{*}(s^\dagger_2,a^\dagger_2) & \cdots & {Q}^{*}(s^\dagger_2, a^\dagger_r)\\
% \vdots & \vdots & \vdots & \vdots\\
% {Q}^*(s_r^\dagger,a^\dagger_1) & {Q}^{*}(s^\dagger_r,a^\dagger_2) & \cdots & {Q}^{*}(s^\dagger_r, a^\dagger_r)
% \end{bmatrix}
% \end{equation*}
% That is, $\mathbb{Q}^{\dagger}$ is the matrix that replaces the entries in $\hat{\mathbb{Q}}^{(t),\dagger}$ with their groudtruth optimal value.
% % \begin{equation*}
% %     {Q}^{*,\dagger} = \begin{bmatrix}
% % {Q}^*(s_1^\dagger,a^\dagger_1) & {Q}^{*}(s^\dagger_1,a^\dagger_2) & \cdots & {Q}^{*}(s^\dagger_1, a^\dagger_r)\\
% % \vdots & \vdots & \vdots & \vdots\\
% % {Q}^*(s_r^\dagger,a^\dagger_1) & {Q}^{*}(s^\dagger_r,a^\dagger_2) & \cdots & {Q}^{*}(s^\dagger_r, a^\dagger_r)
% % \end{bmatrix}
% % \end{equation*}

% \input{alg_rankr}
% \subsection{Theoretical Guarantees}
% \label{subsec:rank2_theory}

% (I think this is not needed: We assume that $R\in[R_{\min}, R_{\max}]$)
% Assume as usual, $|R|\leq R_{\max}$


% \begin{assumption}
% \label{assu:rankr}
% The $r\times r$ matrix $\mathbb{Q}^{\dagger}$ is non-singular.
    
% % \begin{enumerate}
% %     \item The discounting factor $\gamma \leq c\cdot\frac{R_{\min}}{R_{\max}}$.
% %     \item The anchor states $\{s_1^\dagger,s_2^\dagger\}$ and anchor actions $\{a_1^\dagger,a_2^\dagger\}$ satisfy
% %     \begin{equation*}
% %         \frac{Q^*(s_1^\dagger,a_1^\dagger)Q^*(s_2^\dagger,a_2^\dagger)}{Q^*(s_2^\dagger,a_1^\dagger)Q^*(s_1^\dagger,a_2^\dagger)}\geq \frac{(1+c)^2 + \Delta}{(1-c)^2}
% %     \end{equation*}
% %     for some constant $\Delta > 0$.
% % \end{enumerate}
% \end{assumption}

% \begin{lem}
% \label{lem:rankr:unbiased}
% Suppose that Assumption \ref{assu:rankr} holds. Then, for every $(s,a)\in\mS\times\mA$,
% \begin{equation}
% \label{eq:lem:rankr:unbias}
% 		   {Q}^{*}(s,a) = {
% 		    \begin{bmatrix}
% {Q}^{*}(s,a^\dagger_1) &{Q}^{*}(s,a^\dagger_2) &\cdots &{Q}^{*}(s,a^\dagger_r)
% \end{bmatrix}
% \big({\mathbb{Q}}^{\dagger}\big)^{-1}
% % \begin{bmatrix}
% % \hat{Q}^{(t)}(s_2^\dagger,a^\dagger_2) & -\hat{Q}^{(t)}(s^\dagger_1,a^\dagger_2)\\
% % -\hat{Q}^{(t)}(s^\dagger_2,a^\dagger_1) & \hat{Q}^{(t)}(s^\dagger_1,a^\dagger_1)
% % \end{bmatrix}
% \begin{bmatrix}
% {Q}^{*}(s^\dagger_1,a) \\
% {Q}^{*}(s^\dagger_2,a)\\
% \vdots\\
% {Q}^{*}(s^\dagger_r,a)

% \end{bmatrix}
% }
% 		\end{equation}
% \end{lem}

% \begin{prop}
% \label{prop:rankr}
% Fix an iteration $t$ and suppose that Assumption \ref{assu:rankr} holds. If $\forall\:(s,a)\in\Omega^{(t)}$, the estimator $\hat{Q}$ satisfies $|\hat{Q}^{(t)}(s,a)|\leq V_{\max}$ and 
% \begin{equation*}
%     |\hat{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \epsilon,% \:\forall\:(s,a)\in\Omega^{(t)},
% \end{equation*}
% where $\epsilon \leq c{\sigma_{\min}(\mathbb{Q}^{\dagger})}/r$ for some constant $c\in(0,1)$. Then,
% \begin{equation}
%     |\bar{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \eta\cdot \epsilon, \:\forall\:(s,a)\in \mS^{(t)}\times\mA^{(t)},
% \end{equation}
% where $\eta = \frac{r^2V_{\max}}{(1-c)\sigma_{\min}(\mathbb{Q}^\dagger)} \big(2+\frac{rV_{\max}}{\sigma_{\min}(\mathbb{Q}^\dagger)}\big)$.
% \end{prop}
% With Proposition \ref{prop:rankr}, we now have a general-rank matrix estimation oracle that provides a desired entry-wise error bound.
% It is then straightforward to apply our meta theorem, Theorem \ref{thm:generic}, to derive the convergence and sample complexity results for generic rank-$r$ case. We state the main theorem in the following. The proof is again an instantiation of the general proof of Theorem \ref{thm:generic} as have been illustrated for the rank-1 case. For completeness, we provide the proof in xxx
% %with slight modifications following similar logic as in the proof for the rank-1 case. For completeness, 

% % The proof is exactly the same as the one for the rank-1 scenario except that we replace the rank-1 matrix estimation guarantee (Proposition \ref{prop:rank1}) with Proposition \ref{prop:rank2}, in particular, using $\eta = \frac{40R_{\max}^4}{\Delta^2R_{\min}^4}$ in the proof.
% % We hence state the resulting theorem in the following and omit its proof.

% \begin{thm}
% \label{thm:rank-r}
%     %Consider running Algorithm \ref{alg:generic} for $T$ iterations. 
%     Suppose that Assumption \ref{assu:lipschitz} and \ref{assu:rankr} hold. Then, for any MDP problem where $\gamma$ satisfies
%     \begin{equation}
%     \label{eq:thm:rankr:gamma}
%     \gamma <\min\Big\{\frac{c}{r},\:\frac{(1-c)}{r^2\big(2+\frac{rV_{\max}}{\sigma_{\min}(\mathbb{Q}^\dagger)}\big)}\Big\}\cdot \frac{\sigma_{\min}(\mathbb{Q}^\dagger)}{V_{\max}},
%     \end{equation}
%      we have the following guarantees for Algorithm \ref{alg:rank-r}: 
    
%     \begin{enumerate}
%         \item (Convergence) For any $\alpha\in\big(\gamma\frac{r^2V_{\max}}{(1-c)\sigma_{\min}(\mathbb{Q}^\dagger)} \big(2+\frac{rV_{\max}}{\sigma_{\min}(\mathbb{Q}^\dagger)}\big), 1\big)$, there exist appropriate algorithmic parameters such that with probability at least $1-\delta$
%         \begin{equation}
%             |Q^{(T)}(s,a) - Q^*(s,a)|\leq \alpha^TV_{\max},\:\forall\:(s,a)\in\mS\times\mA.
%         \end{equation}
%     \item (Sample Complexity) Therefore, to achieve an $\epsilon$ error for the $Q$-value with probability at least $1-\delta$, i.e., $|Q^{(T)}-Q^*|_{\max}\leq\epsilon$, the number of iterations $T=\Theta\big(\log\frac{1}{\epsilon}\big)$ and the total number of samples needed is
%     \begin{equation}
%         \widetilde{O}\Big(\epsilon^{-(2+d)}\cdot\log\frac{1}{\delta}\Big).
%     \end{equation}
%     \end{enumerate}
% \end{thm}

% \subsection{Proofs}
% \begin{proof}[Proof of Lemma \ref{lem:rankr:unbiased}]
% We use the rank-$r$ assumption, i.e., $Q^*(s,a) = \sum_{i=1}^rf_i(s)g_i(a)$, to expand the R.H.S. of Eq.~(\ref{eq:lem:rankr:unbias}). Denote by
% \begin{align*}
% F^\dagger \triangleq \begin{bmatrix}
% f_1(s^\dagger_1) & f_2(s^\dagger_1) & \cdots & f_r(s^\dagger_1)\\
% f_1(s^\dagger_2) & f_2(s^\dagger_2) & \cdots & f_r(s^\dagger_2)\\
% \vdots & \vdots & \vdots & \vdots\\
% f_1(s^\dagger_r) & f_2(s^\dagger_2) & \cdots & f_r(s^\dagger_r)
% \end{bmatrix}
% \textrm{ and }
% G^\dagger \triangleq \begin{bmatrix}
% g_1(a^\dagger_1) & g_1(a^\dagger_2) & \cdots & g_1(a^\dagger_r)\\
% g_2(a^\dagger_1) & g_2(a^\dagger_2) & \cdots & g_2(a^\dagger_r)\\
% \vdots & \vdots & \vdots & \vdots \\
% g_r(a^\dagger_1) & g_r(a^\dagger_2) & \cdots & g_r(a^\dagger_r)
% \end{bmatrix}.
% \end{align*}
% It is easy to see that $Q^{\dagger} = F^\dagger G^\dagger$. This implies that $ \textrm{rank}(Q^{\dagger})\leq \min\{\textrm{rank}(F^\dagger),\textrm{rank}(G^\dagger)\}$. Since $Q^{\dagger}$ is of rank $r$, and $F^\dagger$ and $G^\dagger$ are both $r\times r$ matrices, the inequality means that both $F^\dagger$ and $G^\dagger$ are full-rank and hence invertible.
% Therefore,
% \begin{align*}
%     \textrm{R.H.S. of Eq.~(\ref{eq:lem:rankr:unbias}) }  &=  \begin{bmatrix}
% {Q}^{*}(s,a^\dagger_1) &{Q}^{*}(s,a^\dagger_2) &\cdots &{Q}^{*}(s,a^\dagger_r)
% \end{bmatrix}
% \big(F^\dagger G^\dagger\big)^{-1}
% \begin{bmatrix}
% {Q}^{*}(s^\dagger_1,a) \\
% {Q}^{*}(s^\dagger_2,a)\\
% \vdots\\
% {Q}^{*}(s^\dagger_r,a)
% \end{bmatrix}\\
% & = 
%     \big(\begin{bmatrix}
%     f_1(s) & f_2(s) & \cdots & f_r(s)
%     \end{bmatrix}G^\dagger\big)(F^\dagger G^\dagger)^{-1}\big(F^\dagger \begin{bmatrix}
%     g_1(a)\\
%     g_2(a)\\
%     \vdots\\
%     g_r(a)
%     \end{bmatrix}\big) \\
%     & = \begin{bmatrix}
%     f_1(s) & f_2(s)& \cdots & f_r(s)
%     \end{bmatrix}G^\dagger (G^\dagger)^{-1}(F^\dagger)^{-1}F^\dagger \begin{bmatrix}
%     g_1(a)\\
%     g_2(a)\\
%     \vdots\\
%     g_r(a)
%     \end{bmatrix}\\
%     & =  \begin{bmatrix}
%     f_1(s) & f_2(s) & \cdots & f_r(s)
%     \end{bmatrix} \begin{bmatrix}
%     g_1(a)\\
%     g_2(a)\\
%     \vdots\\
%     g_r(a)
%     \end{bmatrix}\\
%     & = Q^*(s,a).
% \end{align*}
% This completes the proof of Lemma \ref{lem:rankr:unbiased}.
% \end{proof}

% \begin{proof}[Proof of Proposition \ref{prop:rank2}]
%  Since the context is clear, for simplicity, we omit the superscript $(t)$ for all the notation in the following proof. First, note that by definition of $\bar{Q}$,
%  \begin{equation*}
%      \bar{Q}(s,a)=\sum_{i=1}^r\sum_{j=1}^r \hat{Q}(s,a_i^\dagger)\hat{Q}(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}.
%  \end{equation*}
%  For now, assume that $\hat{\mathbb{Q}}^{\dagger} $ is invertible; we will show later that the condition of Proposition \ref{prop:rankr} guarantees this. Similarly, using Lemma \ref{lem:rankr:unbiased}, we obtain that,
%   \begin{equation*}
%      {Q}^*(s,a)=\sum_{i=1}^r\sum_{j=1}^r {Q}^*(s,a_i^\dagger){Q}^*(s_j^\dagger,a)\big({\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}.
%  \end{equation*}
%  Therefore, 
% \begin{align}
%     |\bar{Q}(s,a) - Q^*(s,a)| &= \Big|\sum_{i=1}^r\sum_{j=1}^r \hat{Q}(s,a_i^\dagger)\hat{Q}(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij} - \sum_{i=1}^r\sum_{j=1}^r {Q}^*(s,a_i^\dagger){Q}^*(s_j^\dagger,a)\big({\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big| \nonumber\\
%     &\leq \sum_{i=1}^r\sum_{j=1}^r\Big|\hat{Q}(s,a_i^\dagger)\hat{Q}(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij} - {Q}^*(s,a_i^\dagger){Q}^*(s_j^\dagger,a)\big({\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big| \nonumber\\
%     & \leq \sum_{i=1}^r\sum_{j=1}^r\bigg(\Big|\hat{Q}(s,a_i^\dagger)\hat{Q}(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij} - {Q}^*(s,a_i^\dagger)\hat{Q}(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big| \nonumber\\ 
%     & \quad \quad\quad\quad+\Big|{Q}^*(s,a_i^\dagger)\hat{Q}(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij} - {Q}^*(s,a_i^\dagger){Q}^*(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big| \nonumber\\
%     & \quad \quad\quad\quad+\Big|{Q}^*(s,a_i^\dagger){Q}^*(s_j^\dagger,a)\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}-  {Q}^*(s,a_i^\dagger){Q}^*(s_j^\dagger,a)\big({\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big|\bigg)\nonumber\\
%     & = \sum_{i=1}^r\sum_{j=1}^r\bigg(\Big|\hat{Q}(s,a_i^\dagger) - Q^*(s,a_i^\dagger)\Big|\cdot \Big|\hat{Q}(s_j^\dagger,a)\Big|\cdot\Big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big| \nonumber\\
%     & \quad \quad\quad\quad+\Big|{Q}^*(s,a_i^\dagger)\Big|\cdot\Big|\hat{Q}(s_j^\dagger,a)-Q^*(s_j^\dagger,a)\Big|\cdot\Big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big|\nonumber\\
%      & \quad \quad\quad\quad+\Big|{Q}^*(s,a_i^\dagger)\Big|\cdot\Big|{Q}^*(s_j^\dagger,a)\Big|\cdot \Big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}_{ij} - \big({\mathbb{Q}}^{\dagger}\big)^{-1}_{ij}\Big|\bigg)\nonumber\\
%      &\leq  \sum_{i=1}^r\sum_{j=1}^r\bigg(\epsilon \cdot V_{\max} \cdot \big|\big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}\big|\big|_{\max} + \epsilon \cdot V_{\max} \cdot \big|\big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}\big|\big|_{\max} \nonumber\\
%     & \quad \quad\quad\quad + V_{\max}^2\cdot\big|\big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1} -\big({\mathbb{Q}}^{\dagger}\big)^{-1} \big|\big|_{\max}\bigg) \label{eq:rankr:prop:diff:ineq}\\
%     & \leq r^2V_{\max}\Big(2\big|\big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}\big|\big|_2\cdot\epsilon + V_{\max}\big|\big|\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1} -\big({\mathbb{Q}}^{\dagger}\big)^{-1} \big|\big|_2\Big ). \label{eq:rankr:prop:proof:bound}
% \end{align} 
% In the above, inequality Eq.~(\ref{eq:rankr:prop:diff:ineq}) follows from the definition of the matrix max norm and the conditions that $|\hat{Q}(s,a)-Q^*(s,a)|\leq \epsilon$ and $|\hat{Q}(s,a)|\leq V_{\max}$. For the last inequality, we use the fact that for a matrix $A$, $||A||_{\max}\leq ||A||_2$.

% To complete the upper bound, in the following, we bound the operator norm of $\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}$ and $\big(\hat{\mathbb{Q}}^{\dagger}\big)^{-1}-\big({\mathbb{Q}}^{\dagger}\big)^{-1}$. To start, we first prove the previous claim that $\hat{\mathbb{Q}}^\dagger$ is invertible. Denote by $\Delta$ the error matrix between  $\hat{\mathbb{Q}}^{\dagger}$ and ${\mathbb{Q}}^{\dagger}$, i.e.,
% \begin{equation*}
%     \Delta = {\mathbb{Q}}^{\dagger} - \hat{\mathbb{Q}}^{\dagger}.
% \end{equation*}
% Note that by assumption, each entry of the matrix $\Delta$ is bounded, in absolute value, by $\epsilon$. Therefore $||\Delta||_2\leq r\epsilon$. Let us now consider $\hat{\mathbb{Q}}^\dagger$.
% \begin{equation*}
%     \hat{\mathbb{Q}}^\dagger = \mathbb{Q}^\dagger -\Delta = \mathbb{Q}^\dagger (\mathbb{I} - (\mathbb{Q}^\dagger)^{-1}\Delta).
% \end{equation*}
% Since the $r\times r$ matrix $ \mathbb{Q}^\dagger$ is invertible, if we show that $\mathbb{I} - (\mathbb{Q}^\dagger)^{-1}\Delta$ is  invertible, then $\hat{\mathbb{Q}}^\dagger$ will be invertible as well. To this end, it suffices to show that $||(\mathbb{Q}^\dagger)^{-1}\Delta||_2 < 1$.
% \begin{align}
%     ||(\mathbb{Q}^\dagger)^{-1}\Delta||_2&\leq ||(\mathbb{Q}^\dagger)^{-1}||_2||\Delta||_2\nonumber\\
%     &\leq \frac{1}{\sigma_{\min}(Q^\dagger)}\cdot r\epsilon \label{eq:rankr:prop:proof:qdelta}\\
%     &\leq c \label{eq:rankr:prop:proof:c},
% \end{align}
% where the last inequality follows from the condition of the proposition that the error $\epsilon $ satisfies $\epsilon \leq c{\sigma_{\min}(\mathbb{Q}^{\dagger})}/r$ for some constant $c\in(0,1)$.

% We are now ready to bound $||(\hat{\mathbb{Q}}^\dagger)^{-1}||_2$.
% \begin{align*}
%     ||(\hat{\mathbb{Q}}^\dagger)^{-1}||_2 &= ||\big(\mathbb{Q}^\dagger (\mathbb{I} - (\mathbb{Q}^\dagger)^{-1}\Delta)\big)^{-1}||_2\\
%     & = ||(\mathbb{I} - (\mathbb{Q}^\dagger)^{-1}\Delta)^{-1} (\mathbb{Q}^\dagger)^{-1}||_2\\
%     & = \Big|\Big|\Big(\sum_{i=0}^\infty \big((\mathbb{Q}^\dagger)^{-1}\Delta\big)^i\Big)(\mathbb{Q}^\dagger)^{-1}\Big|\Big|_2\\
%     &\leq ||(\mathbb{Q}^\dagger)^{-1}||_2 \Big(\sum_{i=0}^\infty \big|\big|(\mathbb{Q}^\dagger)^{-1}\Delta\big|\big|_2^i\Big)\\
%     &\leq \frac{1}{\sigma_{\min}(\mathbb{Q}^\dagger)} \sum_{i=0}^\infty c^i & \textrm{ from Eq.~(\ref{eq:rankr:prop:proof:c})}\\
%     & = \frac{1}{\sigma_{\min}(\mathbb{Q}^\dagger)}\cdot\frac{1}{1-c}
% \end{align*}
% Similarly, we can also bound $||(\hat{\mathbb{Q}}^\dagger)^{-1} - ({\mathbb{Q}}^\dagger)^{-1}||_2$ as follows:
% \begin{align*}
%     ||(\hat{\mathbb{Q}}^\dagger)^{-1}-({\mathbb{Q}}^\dagger)^{-1}||_2 &= ||\big(\mathbb{Q}^\dagger (\mathbb{I} - (\mathbb{Q}^\dagger)^{-1}\Delta)\big)^{-1} - ({\mathbb{Q}}^\dagger)^{-1}||_2\\
%     & = ||(\mathbb{I} - (\mathbb{Q}^\dagger)^{-1}\Delta)^{-1} (\mathbb{Q}^\dagger)^{-1}-({\mathbb{Q}}^\dagger)^{-1}||_2\\
%     & = \Big|\Big|\Big(\sum_{i=0}^\infty \big((\mathbb{Q}^\dagger)^{-1}\Delta\big)^i\Big)(\mathbb{Q}^\dagger)^{-1}-({\mathbb{Q}}^\dagger)^{-1}\Big|\Big|_2\\
%      & = \Big|\Big|\Big(\sum_{i=1}^\infty \big((\mathbb{Q}^\dagger)^{-1}\Delta\big)^i\Big)(\mathbb{Q}^\dagger)^{-1}\Big|\Big|_2\\
%     &\leq ||(\mathbb{Q}^\dagger)^{-1}||_2 ||(\mathbb{Q}^\dagger)^{-1}\Delta||_2\Big(\sum_{i=0}^\infty \big|\big|(\mathbb{Q}^\dagger)^{-1}\Delta\big|\big|_2^i\Big)\\
%     &\leq \frac{1}{\sigma_{\min}(\mathbb{Q}^\dagger)}  ||(\mathbb{Q}^\dagger)^{-1}\Delta||_2 \sum_{i=0}^\infty c^i\\
%     &\leq  \frac{1}{\sigma_{\min}^2(\mathbb{Q}^\dagger)}\cdot\frac{1}{1-c} \cdot r\epsilon & \textrm{ from Eq.~(\ref{eq:rankr:prop:proof:qdelta})}
% \end{align*}
% By applying the upper bounds on $||(\hat{\mathbb{Q}}^\dagger)^{-1}||_2$ and  $||(\hat{\mathbb{Q}}^\dagger)^{-1}-({\mathbb{Q}}^\dagger)^{-1}||_2$ to the previous Eq.~(\ref{eq:rankr:prop:proof:bound}), we final obtain that
% \begin{align*}
%     |\bar{Q}(s,a) - Q^*(s,a)|&\leq r^2V_{\max}\Big(2 \frac{1}{\sigma_{\min}(\mathbb{Q}^\dagger)}\cdot\frac{1}{1-c}\cdot\epsilon + V_{\max}\frac{1}{\sigma_{\min}^2(\mathbb{Q}^\dagger)}\cdot\frac{1}{1-c} \cdot r\epsilon \Big)\\
%     & = \frac{r^2V_{\max}}{(1-c)\sigma_{\min}(\mathbb{Q}^\dagger)} \Big(2+\frac{rV_{\max}}{\sigma_{\min}(\mathbb{Q}^\dagger)}\Big)\cdot \epsilon.
% \end{align*}
% \end{proof}

% \begin{proof}[Proof of Theorem \ref{thm:rank-r}]
%  As mentioned, the proof is basically an instantiation of the generic proof for Theorem \ref{thm:generic}; we replace the assumption on the matrix estimation oracle (i.e., Assumption \ref{assu:me}) with the explicit guarantee obtained in Proposition \ref{prop:rankr}. Similar to the rank-1 case, however, Proposition \ref{prop:rankr} holds only when the error $|\hat{Q}^{(t)}(s,a)-Q^*(s,a)|$ satisfies certain condition. 
%  We will hence modify few key steps of the generic proof, following the same logic as we have illustrated in the proof of the rank-1 case. Again, eventually, the only difference of those modifications are that our choices of algorithmic parameters change slightly. Most of the proof below follows closely the proof of the rank-1 case. We include it here for completeness.
 
% Recall Part I of the generic proof and fix an iteration $t$. Suppose that the error of $\hat{V}^{(t-1)}$ satisfies that 
% $||\hat{V}^{(t-1)}-V^*||_{\max} \leq B^{(t-1)}.$ Then, by applying Lemma \ref{lem:one_step_lookahead}, we obtain that 
% for a state-action pair $(s,a)\in\Omega^{(t)}$, with probability $1- \xi$, the improve estimate $\hat{Q}^{(t)}(s,a)$ from simple lookahead simulations satisfies
% \begin{equation*}
% %\label{eq:proof:thm:generic:one_step}
%     |\hat{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \gamma(\lambda^{(t)} + B^{(t-1)}).
% \end{equation*}
%  For now, let us also assume that the bound $B^{(t-1)}$ satisfies $B^{(t-1)}\leq V_{\max}$; we will see that this is easily implied by our choices of algorithmic parameters. Then, from the condition of Theorem \ref{thm:rank-r}, i.e., Eq.~(\ref{eq:thm:rankr:gamma}) on $\gamma$, $\frac{c\sigma_{\min}(\mathbb{Q}^\dagger)}{r\gamma}-V_{\max} > 0$. It is hence obvious that if we let 
% \begin{equation*}
%     \lambda ^{(t)}\leq \frac{c\sigma_{\min}(\mathbb{Q}^\dagger)}{r\gamma}-V_{\max},
% \end{equation*}
% we have the following error guarantee
% \begin{equation*}
% %\label{eq:proof:thm:generic:one_step}
%     |\hat{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \gamma(\lambda^{(t)} + B^{(t-1)})\leq \frac{c\sigma_{\min}(\mathbb{Q}^\dagger)}{r}.
% \end{equation*}
% In particular, note that this allows us to apply Proposition \ref{prop:rankr} to derive the error bound for $\bar{Q}^{(t)}$ after the matrix completion step. In the subsequent proof, we will condition on that $\lambda^{(t)}$ is selected such that  $\lambda ^{(t)}\leq \frac{c\sigma_{\min}(\mathbb{Q}^\dagger)}{r\gamma}-V_{\max}$ for all $t=1,\dots,T$. Therefore, we obtain that at iteration $t$, with probability at least $1-|\Omega^{(t)}|\times\xi$,
% \begin{equation*}
%     |\bar{Q}^{(t)}(s,a) - Q^*(s,a)|\leq \gamma\eta(\lambda^{(t)}+B^{(t-1)}), \:\forall\:(s,a)\in\mS^{(t)} \times \mA^{(t)},
% \end{equation*}
% where 
% \begin{equation*}
%     \eta =  \frac{r^2V_{\max}}{(1-c)\sigma_{\min}(\mathbb{Q}^\dagger)} \big(2+\frac{rV_{\max}}{\sigma_{\min}(\mathbb{Q}^\dagger)}\big).
% \end{equation*}
% Finally, note that in Algorithm \ref{alg:rank-r}, $\Omega^{(t)} = \big\{(s^\dagger, a)\big\}_{s^\dagger\in\{s^\dagger_1,s^\dagger_2,\dots, s^\dagger_r\},a\in\mA^{(t)}}  \bigcup \{(s, a^\dagger_1)\big\}_{{s\in\mS^{(t)}},{a^\dagger\in\{a^\dagger_1,a^\dagger_2,\dots, a^\dagger_r\}}}$. Hence, we have that $|\Omega^{(t)}|=O\big(2r(|\mS^{(t)}|\vee|\mA^{(t)}|)\big) = O\big((\beta^{(t)})^{-d})$.

% For Part II of the generic proof, it is obvious that the recursive equation readily follows. Precisely, using the same definitions of $\varepsilon^{(t)}_Q$ and $\varepsilon^{(t)}_V$,
% \begin{align}
% \label{eq:thm:rankr:proof:recursion}
%   \varepsilon^{(t)}_Q 
%     & \leq  2L\beta^{(t)} + \gamma\eta\lambda^{(t)} + \gamma\eta \varepsilon_Q^{(t-1)} .
% \end{align}

% To select the algorithmic parameters, we follow the same reasoning as in Part III of the generic proof. Specifically, we prove by induction that for every $ t= 0, 1,2,\dots, T$
% \begin{equation}
% \label{eq:thm:rankr:proof:induction}
%     \varepsilon^{(t)}_Q\leq V_{\max}\alpha^t,
% \end{equation}
% where we recall that $\alpha\in\big(\gamma\frac{r^2V_{\max}}{(1-c)\sigma_{\min}(\mathbb{Q}^\dagger)} \big(2+\frac{rV_{\max}}{\sigma_{\min}(\mathbb{Q}^\dagger)}\big), 1\big)$ and that the condition Eq.~(\ref{eq:thm:rankr:gamma}) on $\gamma$ guarantees the previous interval is non-empty.
% Note that Eq.~(\ref{eq:thm:rankr:proof:induction}) would lead to the desired convergence result in Theorem \ref{thm:rank-r}. In addition, by using the fact that $\varepsilon^{(t)}_V\leq \varepsilon^{(t)}_Q$ (cf. Eq.~(\ref{eq:thm:generic:proof:varepsilonV})), the above equation also implies that $B^{(t)}\leq V_{\max}$ for each iteration $t$, which is desirable as mentioned previously. 

% Let us prove the result Eq.~(\ref{eq:thm:rankr:proof:induction}) by induction. Notice that $\varepsilon^{(0)}_Q\leq V_{\max}$ holds trivially by setting $Q^{(0)}=0$. By induction, suppose that  $\varepsilon^{(t-1)}_Q\leq V_{\max}\alpha^{t-1}$, then from the recursive equation Eq.~(\ref{eq:thm:rankr:proof:recursion}), we would like to show that we could choose appropriate parameters such that
% \begin{align*}
%     \varepsilon^{(t)}_Q&\leq  2L\beta^{(t)} + \gamma\eta\lambda^{(t)} + \gamma\eta V_{\max}\alpha^{t-1} \nonumber\\
%     &\leq V_{\max}\alpha^{t}.
% \end{align*}
% Again, it is not hard to see that one could set the parameters $\beta^{(t)}$ and $\lambda^{(t)}$ to be such that
% \begin{align*}
%     2L\beta^{(t)} \leq \frac{\alpha-\gamma\eta}{2}V_{\max}\alpha^{t-1}\textrm{ and }\gamma\eta\lambda^{(t)}  \leq \frac{\alpha-\gamma\eta}{2}V_{\max}\alpha^{t-1}.
% \end{align*}
% Additionally, recall that previously in the proof, to apply Proposition \ref{prop:rankr} for the matrix estimation step, we have conditioned on that $\lambda^{(t)}$ is selected such that  $\lambda ^{(t)}\leq \frac{c\sigma_{\min}(\mathbb{Q}^\dagger)}{r\gamma}-V_{\max}$ for each iteration $t$. Therefore, to summarize, we can set the parameters to be 
% \begin{align}
%     \beta^{(t)} = \frac{\alpha-\gamma\eta}{4L}V_{\max}\alpha^{t-1}\textrm{ and }\lambda^{(t)}  = \min\Big\{\frac{c\sigma_{\min}(\mathbb{Q}^\dagger)}{r\gamma}-V_{\max}, \frac{\alpha-\gamma\eta}{2\gamma\eta}V_{\max}\alpha^{t-1}\Big\}. \label{eq:thm:rankr:proof:constants}
% \end{align}
% With these choices of $\beta^{(t)}$ and $\lambda^{(t)}$, we complete the induction proof that $\varepsilon^{(t)}_Q\leq V_{\max}\alpha^t$.

% Finally, the sample complexity follows exactly the same steps in Part IV of the generic proof. In particular, we note that to achieve $\varepsilon^{(T)}_Q\leq \epsilon$, we have $T=\Theta(\log\frac{1}{\epsilon})$ from the induction proof above. Furthermore, the choice of $\beta^{(t)}$ and $\lambda^{(t)}$ in Eq.~(\ref{eq:thm:rankr:proof:constants}) implies that $\beta^{(T)}=\Theta(\epsilon)$ and $\lambda^{(T)}=\Theta(\epsilon)$. The rest of the calculation for sample complexity is exactly the same, and this completes the proof of Theorem \ref{thm:rank-r}.
% \end{proof}
